A Continual Learning-driven Model for Accurate and Generalizable Segmentation of Clinically Comprehensive and Fine-grained Whole-body Anatomies in CT

Precision medicine in the quantitative management of chronic diseases and oncology would be greatly improved if the Computed Tomography (CT) scan of any patient could be segmented, parsed and analyzed in a precise and detailed way. However, there is no such fully annotated CT dataset with all anatomies delineated for training because of the exceptionally high manual cost, the need for specialized clinical expertise, and the time required to finish the task. To this end, we proposed a novel continual learning-driven CT model that can segment complete anatomies presented using dozens of previously partially labeled datasets, dynamically expanding its capacity to segment new ones without compromising previously learned organ knowledge. Existing multi-dataset approaches are not able to dynamically segment new anatomies without catastrophic forgetting and would encounter optimization difficulty or infeasibility when segmenting hundreds of anatomies across the whole range of body regions. Our single unified CT segmentation model, CL-Net, can highly accurately segment a clinically comprehensive set of 235 fine-grained whole-body anatomies. Composed of a universal encoder, multiple optimized and pruned decoders, CL-Net is developed using 13,952 CT scans from 20 public and 16 private high-quality partially labeled CT datasets of various vendors, different contrast phases, and pathologies. Extensive evaluation demonstrates that CL-Net consistently outperforms the upper limit of an ensemble of 36 specialist nnUNets trained per dataset with the complexity of 5% model size and significantly surpasses the segmentation accuracy of recent leading Segment Anything-style medical image foundation models by large margins. Our continual learning-driven CL-Net model would lay a solid foundation to facilitate many downstream tasks of oncology and chronic diseases using the most widely adopted CT imaging.

==> Tabs/tab_abbr2.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ll}
\hline
\multicolumn{1}{l}{Model} & \multicolumn{1}{c}{Definition} \\ \hline
\ac{cln_c5} & Default \ac{clnet} (w. pruning and \acs{fls}) trained using five representative datasets under \acs{css} setup \\
\ac{cln_unprn} & \ac{clnet} trained w.o. pruning using five representative datasets under \acs{css} setup \\
\ac{cln_u5} & Default \ac{clnet} trained using five representative datasets under Universal Segmentation setup \\
\ac{nnu_e5} & Ensemble of five nnUNet specialists trained using five representative datasets \\ \hline
\ac{cln_c36} & Default \ac{clnet} trained using the full 36 internal datasets under \acs{css} setup \\
\ac{cln_u36} & Default \ac{clnet} trained using the full 36 internal datasets under Universal Segmentation setup \\
\ac{cln_u36_unprn} & \ac{clnet} trained w.o. pruning using the full 36 internal datasets under Universal Segmentation setup \\
\ac{cln_c36_nofls} & \ac{clnet} trained w.o. pruning or \acs{fls} using the full 36 internal datasets under \acs{css} setup \\
\ac{cln_u36_nofls} & \ac{clnet} trained w.o. pruning or \acs{fls} using the full 36 internal datasets under Universal Segmentation setup \\
\ac{cln_u36_ft} & \ac{cln_u36} fine-tuned on five representative datasets \\
\ac{nnu_e36} & Ensemble of 36 nnUNet specialists trained using the full 36 internal datasets \\ \hline
\end{tabular}
}
\caption{\textbar~\textbf{List of Models.}}
\label{tab:abbr}
\end{table}

==> Tabs/tabs_ds36_uni/tab_uni_avg.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{|l|ll|ll|ll|}
\hline
 & \multicolumn{2}{c|}{\textbf{SUNSeg$^{\mathcal{C}_{36}}$}} & \multicolumn{2}{c|}{\textbf{SUNSeg$^{\mathcal{U}_{36}}$}} & \multicolumn{2}{c|}{\textbf{nnUNet$^{E_{36}}$}} \\ \cline{2-7} 
 & DSC$\uparrow$              & ASD$\downarrow$              & DSC$\uparrow$              & ASD$\downarrow$              & DSC$\uparrow$         & ASD$\downarrow$         \\ \hline
Head \& Neck (49) & 79.60  & 1.01 & 80.64 & 0.95 & 74.26 & 1.18 \\
Chest (52)        & 88.03 & 1.19 & 88.15 & 1.17 & 85.45 & 1.37 \\
Abdomen (28)      & 91.51 & 1.02 & 91.84 & 0.97 & 90.81 & 1.14 \\
Bone (63)         & 92.14 & 0.83 & 92.28 & 0.82 & 91.92 & 0.86 \\
LNS (33)          & 72.23 & 1.30  & 72.27 & 1.29 & 72.11 & 1.35 \\
Lesion (10)       & 70.67 & 3.67 & 70.89 & 3.48 & 70.31 & 3.59 \\
Body (1)          & 97.09 & 2.33 & 97.11 & 2.51 & 96.97 & 2.20  \\ \hline
All               & 84.89 & 1.16 & 85.22 & 1.13 & 83.03 & 1.26 \\ \hline
\end{tabular}%
}
\caption{Full-scale \ac{clnet} organ-group-wise performance: the mean DSC and ASD of SUNSeg$^{\mathcal{C}_{36}}$ and SUNSeg$^{\mathcal{U}_{36}}$. nnUNet$^{E_{36}}$ is used as segmentation upper bound. The organ number of each group is annotated after the organ group name. }
\label{tab:ds36_res_avg}
\end{table}

==> Tabs/tabs_ds36_uni/tab_uni_prune.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccc|cc|}
\hline
 & \multicolumn{4}{c|}{\textbf{SUNSeg$^{\mathcal{U}_{36}}$}}                    & \multicolumn{2}{c|}{\textbf{SUNSeg$^{\mathcal{U}_{36}}_{\text{unpruned}}$}} \\ \cline{2-7} 
 & DSC$\uparrow$ & ASD$\downarrow$ & $\mathcal{T}$$\uparrow$ & Decoder Size (M) & DSC$\uparrow$                       & ASD$\downarrow$                       \\ \hline
Head \& Neck (28) & 81.23 & 0.95 & 97.25 & 12.1 & 81.22 & 0.96 \\
Chest (31)        & 87.83 & 1.12 & 98.58 & 6.9  & 87.83 & 1.13 \\
Abdomen (19)      & 91.09 & 1.13 & 98.84 & 3.5  & 91.10  & 1.14 \\
Bone (11)         & 93.02 & 1.10  & 98.83 & 2.0  & 93.01 & 1.11 \\
LNS (2)           & 72.52 & 1.28 & 88.00    & 3.8  & 72.52 & 1.29 \\
Lesion (10)       & 70.89 & 3.48 & 92.60  & 11.6 & 70.81 & 3.65 \\ \hline
All               & 85.20 & 1.31 & 97.48 & 39.8 & 85.19 & 1.33 \\ \hline
\end{tabular}%
}
\caption{Full-scale \ac{clnet} organ-group-wise decoder performance: the mean DSC and ASD of the decoders in each organ group of the pruned and unpruned SUNSeg$^{\mathcal{U}_{36}}$. The mean pruning rate and total decoder size of SUNSeg$^{\mathcal{U}_{36}}$ in each group is also provided. The decoder number of each organ group is annotated after the group name. }
\label{tab:ds36_prune_avg}
\end{table}

==> Tabs/tabs_ds5_pl/tab_pl_flare.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
Liver & 98.1$\pm$14.5 & 0.83$\pm$0.98 & 97.5$\pm$5.6 & 0.80$\pm$0.99 & 97.3$\pm$3.4 & 0.74$\pm$1.11 & 94.9$\pm$5.8 & 0.81$\pm$1.00 & 99.5 & 93.7$\pm$5.9 & 0.81$\pm$0.95 & 99.5 & 95.0$\pm$5.6 & 0.79$\pm$0.99 & 99.5 \\
Kidney\_R & 92.4$\pm$16.9 & 1.81$\pm$0.74 & 92.7$\pm$6.8 & 1.20$\pm$0.73 & 94.3$\pm$9.2 & 3.40$\pm$9.09 & 94.3$\pm$7.1 & 1.44$\pm$0.76 & 99.7 & 95.0$\pm$7.0 & 1.78$\pm$0.75 & 99.7 & 94.4$\pm$7.0 & 1.36$\pm$0.75 & 99.7 \\
Kidney\_L & 92.8$\pm$16.9 & 1.27$\pm$0.74 & 90.8$\pm$6.7 & 1.51$\pm$0.70 & 97.1$\pm$3.4 & 0.45$\pm$0.89 & 92.1$\pm$6.7 & 1.18$\pm$0.69 & {} & 91.1$\pm$6.7 & 1.29$\pm$0.70 & {} & 94.3$\pm$6.9 & 1.06$\pm$0.72 & {} \\
\rowcolor[HTML]{F3F3F3} 
Spleen & 97.9$\pm$15.6 & 0.30$\pm$0.37 & 97.0$\pm$6.9 & 0.20$\pm$0.40 & 89.0$\pm$4.8 & 0.98$\pm$0.68 & 98.0$\pm$6.6 & 0.19$\pm$0.37 & 99.5 & 98.0$\pm$6.7 & 0.32$\pm$0.39 & 99.5 & 98.1$\pm$6.9 & 0.20$\pm$0.40 & 99.5 \\
Pancreas & 91.6$\pm$17.2 & 0.80$\pm$0.69 & 87.9$\pm$7.1 & 0.71$\pm$0.39 & 94.5$\pm$8.0 & 1.58$\pm$3.43 & 92.4$\pm$7.0 & 0.72$\pm$0.38 & 99.5 & 94.9$\pm$7.0 & 0.86$\pm$0.38 & 99.5 & 92.6$\pm$7.0 & 0.74$\pm$0.38 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
A\_Aorta & 96.7$\pm$16.5 & 0.21$\pm$0.95 & 94.2$\pm$16.7 & 0.96$\pm$0.85 & 90.3$\pm$10.2 & 0.83$\pm$1.11 & 97.1$\pm$16.5 & 0.18$\pm$0.83 & 99.7 & 92.2$\pm$16.7 & 0.23$\pm$0.85 & 99.0 & 97.1$\pm$16.6 & 0.18$\pm$0.84 & 99.5 \\
V\_VenaCava\_I & 89.8$\pm$10.1 & 1.08$\pm$1.03 & 83.2$\pm$10.2 & 1.48$\pm$1.01 & 84.3$\pm$7.0 & 0.44$\pm$0.53 & 88.6$\pm$9.9 & 1.12$\pm$0.98 & 99.0 & 78.5$\pm$10.0 & 1.17$\pm$1.02 & 99.0 & 88.8$\pm$9.9 & 1.08$\pm$0.97 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
Glnd\_Adrenal\_R & 85.9$\pm$12.3 & 0.39$\pm$0.37 & 86.9$\pm$13.3 & 0.39$\pm$0.39 & 85.9$\pm$6.1 & 0.34$\pm$0.19 & 87.9$\pm$13.2 & 0.35$\pm$0.39 & 96.0 & 90.3$\pm$13.4 & 0.43$\pm$0.41 & 98.0 & 89.0$\pm$13.2 & 0.33$\pm$0.39 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
Glnd\_Adrenal\_L & 88.0$\pm$13.3 & 0.26$\pm$1.16 & 86.3$\pm$12.4 & 0.32$\pm$0.37 & 81.0$\pm$23.4 & 2.06$\pm$2.84 & 87.7$\pm$12.5 & 0.21$\pm$0.38 & {\cellcolor[HTML]{F3F3F3}} & 87.6$\pm$12.5 & 0.28$\pm$0.39 & {\cellcolor[HTML]{F3F3F3}} & 89.9$\pm$12.6 & 0.22$\pm$0.39 & {\cellcolor[HTML]{F3F3F3}} \\
GallBladder & 80.2$\pm$24.7 & 2.16$\pm$0.83 & 80.1$\pm$8.4 & 2.22$\pm$0.80 & 84.1$\pm$15.4 & 1.93$\pm$3.34 & 83.1$\pm$8.7 & 2.12$\pm$0.83 & 99.5 & 85.5$\pm$8.4 & 2.15$\pm$0.80 & 99.5 & 83.2$\pm$8.5 & 2.27$\pm$0.82 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Eso & 84.4$\pm$3.1 & 1.70$\pm$0.15 & 85.9$\pm$2.9 & 0.70$\pm$0.14 & 89.8$\pm$19.8 & 2.09$\pm$4.22 & 86.0$\pm$3.0 & 1.61$\pm$0.14 & 99.7 & 81.8$\pm$3.2 & 1.66$\pm$0.16 & 98.0 & 86.1$\pm$2.8 & 1.50$\pm$0.13 & 99.5 \\
Stomach & 91.7$\pm$16.4 & 1.24$\pm$0.67 & 91.0$\pm$6.4 & 1.28$\pm$0.68 & 79.0$\pm$16.9 & 4.77$\pm$8.97 & 92.4$\pm$6.5 & 1.17$\pm$0.69 & 99.5 & 92.3$\pm$6.5 & 1.17$\pm$0.68 & 99.5 & 92.5$\pm$6.2 & 1.05$\pm$0.65 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Duodenum & 79.8$\pm$25.9 & 2.71$\pm$1.29 & 76.6$\pm$15.9 & 2.59$\pm$1.29 & 94.2$\pm$9.6 & 4.22$\pm$8.64 & 81.0$\pm$16.1 & 2.39$\pm$1.18 & 99.5 & 82.6$\pm$15.9 & 2.60$\pm$1.26 & 99.5 & 83.2$\pm$15.8 & 2.36$\pm$1.19 & 99.5
\\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise FLARE22}
\end{table}

==> Tabs/tabs_ds5_pl/tab_pl_kits.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
Kidney \Ac{gtv} & 86.7$\pm$9.0 & 1.18$\pm$1.06 & 83.7$\pm$9.2 & 1.10$\pm$1.08 & 79.6$\pm$20.8 & 9.94$\pm$17.66 & 87.2$\pm$9.0 & 1.03$\pm$0.98 & 96.0 & 83.9$\pm$9.0 & 1.18$\pm$1.04 & 90.0 & 87.1$\pm$9.4 & 1.28$\pm$1.05 & 96.0

\\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise KiTS21 }
\end{table}

==> Tabs/tabs_ds5_pl/tab_pl_segthor.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
Eso & 88.2$\pm$3.2 & 0.35$\pm$0.16 & 86.0$\pm$3.2 & 0.66$\pm$0.16 & 83.1$\pm$8.5 & 1.17$\pm$0.98 & 90.4$\pm$3.0 & 0.31$\pm$0.14 & 99.5 & 89.9$\pm$2.8 & 0.53$\pm$0.12 & 98.0 & 90.5$\pm$2.9 & 0.32$\pm$0.13 & 99.5 \\
Heart & 94.7$\pm$14.9 & 0.39$\pm$0.20 & 94.2$\pm$14.6 & 1.62$\pm$0.18 & 94.3$\pm$1.0 & 3.44$\pm$3.79 & 94.5$\pm$14.6 & 0.37$\pm$0.17 & 99.0 & 91.4$\pm$14.8 & 1.48$\pm$0.19 & 99.0 & 94.6$\pm$14.6 & 0.37$\pm$0.18 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
Trachea & 92.2$\pm$5.8 & 0.30$\pm$0.09 & 90.4$\pm$6.0 & 0.78$\pm$0.11 & 90.7$\pm$3.5 & 0.67$\pm$0.39 & 93.8$\pm$5.9 & 0.28$\pm$0.10 & 99.5 & 92.7$\pm$6.1 & 0.68$\pm$0.12 & 99.7 & 92.9$\pm$5.8 & 0.31$\pm$0.09 & 99.5 \\
A\_Aorta & 95.2$\pm$16.6 & 0.32$\pm$0.84 & 94.3$\pm$16.5 & 0.90$\pm$0.82 & 94.6$\pm$0.8 & 0.47$\pm$0.11 & 96.2$\pm$16.6 & 0.31$\pm$0.84 & 99.7 & 95.3$\pm$16.8 & 0.75$\pm$0.86 & 99.0 & 95.9$\pm$16.7 & 0.34$\pm$0.85 & 99.5
\\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise SegTHOR }
\end{table}

==> Tabs/tabs_ds5_pl/tab_pl_structseg.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{31}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
BrainStem & 93.7$\pm$1.5 & 0.32$\pm$0.10 & 91.2$\pm$1.5 & 0.80$\pm$0.10 & 87.2$\pm$2.5 & 0.84$\pm$0.26 & 92.9$\pm$1.6 & 0.23$\pm$0.11 & 99.5 & 93.6$\pm$1.7 & 0.76$\pm$0.11 & 99.5 & 93.1$\pm$1.7 & 0.24$\pm$0.12 & 99.0 \\
Eye\_L & 94.8$\pm$1.3 & 0.17$\pm$0.08 & 85.7$\pm$1.2 & 0.82$\pm$0.07 & 89.5$\pm$2.9 & 0.40$\pm$0.12 & 93.6$\pm$1.3 & 0.14$\pm$0.08 & 99.0 & 86.6$\pm$1.4 & 0.69$\pm$0.09 & 99.0 & 93.7$\pm$1.3 & 0.13$\pm$0.08 & 99.0 \\
Eye\_R & 93.2$\pm$4.2 & 0.24$\pm$0.28 & 87.7$\pm$4.0 & 0.55$\pm$0.27 & 90.0$\pm$2.5 & 1.43$\pm$2.58 & 95.3$\pm$4.3 & 0.28$\pm$0.29 & {} & 86.7$\pm$4.3 & 0.57$\pm$0.29 & {} & 95.4$\pm$4.3 & 0.25$\pm$0.29 & {} \\
\rowcolor[HTML]{F3F3F3} 
Lens\_L & 80.1$\pm$9.8 & 0.25$\pm$0.18 & 78.6$\pm$9.8 & 0.57$\pm$0.18 & 77.9$\pm$6.3 & 0.23$\pm$0.14 & 80.4$\pm$9.8 & 0.21$\pm$0.17 & 96.0 & 81.6$\pm$9.9 & 0.56$\pm$0.18 & 99.0 & 82.5$\pm$9.9 & 0.22$\pm$0.19 & 98.0 \\
\rowcolor[HTML]{F3F3F3} 
Lens\_R & 79.7$\pm$9.2 & 0.33$\pm$0.43 & 80.4$\pm$9.2 & 0.48$\pm$0.42 & 80.3$\pm$5.6 & 0.21$\pm$0.09 & 82.0$\pm$9.3 & 0.41$\pm$0.43 & {\cellcolor[HTML]{F3F3F3}} & 84.3$\pm$9.4 & 0.37$\pm$0.44 & {\cellcolor[HTML]{F3F3F3}} & 82.1$\pm$9.3 & 0.43$\pm$0.43 & {\cellcolor[HTML]{F3F3F3}} \\
OpticNerve\_L & 80.3$\pm$8.0 & 0.29$\pm$0.28 & 67.6$\pm$8.1 & 0.78$\pm$0.30 & 67.3$\pm$8.7 & 1.11$\pm$1.78 & 81.7$\pm$8.1 & 0.31$\pm$0.30 & 99.0 & 77.8$\pm$8.0 & 0.60$\pm$0.28 & 99.0 & 80.8$\pm$8.0 & 0.33$\pm$0.29 & 99.5 \\
OpticNerve\_R & 84.1$\pm$6.4 & 0.20$\pm$0.21 & 66.8$\pm$6.5 & 0.81$\pm$0.22 & 68.1$\pm$7.0 & 0.52$\pm$0.15 & 86.5$\pm$6.2 & 0.17$\pm$0.20 & {} & 79.3$\pm$6.1 & 0.59$\pm$0.19 & {} & 81.6$\pm$6.2 & 0.19$\pm$0.20 & {} \\
\rowcolor[HTML]{F3F3F3} 
Chiasm & 71.6$\pm$12.9 & 0.26$\pm$0.13 & 48.5$\pm$12.8 & 1.42$\pm$0.12 & 42.9$\pm$18.6 & 23.27$\pm$47.95 & 71.9$\pm$13.1 & 0.23$\pm$0.15 & 96.0 & 74.5$\pm$13.0 & 0.62$\pm$0.14 & 96.0 & 69.1$\pm$13.3 & 0.29$\pm$0.16 & 99.5 \\
TemporalLobe\_L & 94.7$\pm$1.2 & 0.24$\pm$0.08 & 90.4$\pm$1.3 & 2.18$\pm$0.09 & 85.6$\pm$7.0 & 1.93$\pm$0.94 & 95.3$\pm$1.3 & 0.22$\pm$0.09 & 99.5 & 88.2$\pm$1.3 & 1.41$\pm$0.09 & 99.5 & 95.5$\pm$1.1 & 0.20$\pm$0.07 & 99.7 \\
TemporalLobe\_R & 94.8$\pm$1.4 & 0.26$\pm$0.09 & 92.7$\pm$1.4 & 2.26$\pm$0.09 & 84.1$\pm$6.0 & 2.02$\pm$0.83 & 93.5$\pm$1.6 & 0.23$\pm$0.11 & {} & 87.6$\pm$1.7 & 1.73$\pm$0.13 & {} & 95.7$\pm$1.5 & 0.25$\pm$0.10 & {} \\
\rowcolor[HTML]{F3F3F3} 
Glnd\_Pituitary & 84.5$\pm$6.4 & 0.22$\pm$0.21 & 65.0$\pm$6.5 & 1.01$\pm$0.22 & 52.6$\pm$23.3 & 1.04$\pm$0.65 & 85.6$\pm$6.4 & 0.16$\pm$0.21 & 99.0 & 85.2$\pm$6.5 & 0.49$\pm$0.21 & 98.0 & 88.7$\pm$6.3 & 0.15$\pm$0.20 & 99.5 \\
Glnd\_Parotid\_L & 93.3$\pm$1.9 & 0.35$\pm$0.16 & 85.6$\pm$1.9 & 1.05$\pm$0.16 & 83.0$\pm$5.6 & 1.19$\pm$0.58 & 91.7$\pm$1.7 & 0.29$\pm$0.15 & 99.5 & 87.6$\pm$1.7 & 1.06$\pm$0.14 & 99.5 & 95.9$\pm$1.9 & 0.30$\pm$0.16 & 99.5 \\
Glnd\_Parotid\_R & 92.5$\pm$3.4 & 0.50$\pm$0.52 & 85.7$\pm$3.5 & 1.09$\pm$0.53 & 84.3$\pm$4.4 & 1.20$\pm$0.55 & 96.0$\pm$1.3 & 0.42$\pm$0.50 & {} & 86.6$\pm$1.4 & 1.09$\pm$0.51 & {} & 96.1$\pm$1.4 & 0.41$\pm$0.52 & {} \\
\rowcolor[HTML]{F3F3F3} 
Ear\_Inner\_L & 67.0$\pm$9.5 & 0.66$\pm$0.37 & 67.6$\pm$9.6 & 1.09$\pm$0.39 & 83.1$\pm$2.7 & 0.50$\pm$0.12 & 69.3$\pm$9.4 & 0.61$\pm$0.36 & 99.5 & 58.3$\pm$9.5 & 0.60$\pm$0.37 & 99.5 & 65.5$\pm$9.3 & 0.61$\pm$0.35 & 98.0 \\
\rowcolor[HTML]{F3F3F3} 
Ear\_Inner\_R & 64.3$\pm$9.3 & 0.66$\pm$0.30 & 66.8$\pm$9.1 & 0.60$\pm$0.29 & 86.8$\pm$2.7 & 0.33$\pm$0.11 & 63.8$\pm$9.4 & 0.75$\pm$0.31 & {\cellcolor[HTML]{F3F3F3}} & 57.1$\pm$9.4 & 0.57$\pm$0.32 & {\cellcolor[HTML]{F3F3F3}} & 65.0$\pm$9.4 & 0.79$\pm$0.32 & {\cellcolor[HTML]{F3F3F3}} \\
Ear\_Mid\_L & 90.4$\pm$3.7 & 0.07$\pm$0.04 & 80.1$\pm$3.8 & 0.97$\pm$0.05 & 75.2$\pm$15.7 & 1.30$\pm$1.14 & 90.6$\pm$3.6 & 0.07$\pm$0.03 & 99.5 & 91.3$\pm$3.7 & 0.57$\pm$0.04 & 99.5 & 90.7$\pm$3.6 & 0.07$\pm$0.02 & 99.7 \\
Ear\_Mid\_R & 90.2$\pm$3.3 & 0.08$\pm$0.06 & 80.0$\pm$3.2 & 0.94$\pm$0.05 & 81.2$\pm$7.0 & 1.69$\pm$2.60 & 92.1$\pm$3.4 & 0.07$\pm$0.06 & {} & 90.4$\pm$3.4 & 0.64$\pm$0.06 & {} & 89.2$\pm$3.3 & 0.07$\pm$0.05 & {} \\
\rowcolor[HTML]{F3F3F3} 
TMJ\_L & 84.4$\pm$9.5 & 0.31$\pm$0.23 & 77.2$\pm$9.4 & 0.65$\pm$0.23 & 78.1$\pm$6.8 & 0.79$\pm$0.34 & 82.5$\pm$9.3 & 0.24$\pm$0.22 & 98.0 & 78.6$\pm$9.4 & 0.65$\pm$0.23 & 94.0 & 78.7$\pm$9.5 & 0.36$\pm$0.23 & 96.0 \\
\rowcolor[HTML]{F3F3F3} 
TMJ\_R & 84.1$\pm$7.6 & 0.33$\pm$0.20 & 75.2$\pm$7.4 & 0.75$\pm$0.18 & 75.8$\pm$6.7 & 1.55$\pm$2.24 & 84.3$\pm$7.7 & 0.33$\pm$0.21 & {\cellcolor[HTML]{F3F3F3}} & 76.8$\pm$7.9 & 0.71$\pm$0.23 & {\cellcolor[HTML]{F3F3F3}} & 80.5$\pm$7.5 & 0.37$\pm$0.20 & {\cellcolor[HTML]{F3F3F3}} \\
SpinalCord & 91.5$\pm$2.9 & 0.36$\pm$0.19 & 91.7$\pm$3.1 & 0.86$\pm$0.20 & 81.4$\pm$3.2 & 0.61$\pm$0.14 & 90.8$\pm$3.1 & 0.33$\pm$0.21 & 99.0 & 94.4$\pm$3.0 & 0.67$\pm$0.20 & 99.7 & 94.9$\pm$3.2 & 0.35$\pm$0.22 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Mandible\_L & 95.7$\pm$2.1 & 0.17$\pm$0.08 & 94.2$\pm$2.0 & 0.50$\pm$0.06 & 91.4$\pm$1.9 & 0.37$\pm$0.13 & 97.5$\pm$2.0 & 0.15$\pm$0.07 & 99.7 & 92.2$\pm$1.8 & 0.43$\pm$0.05 & 99.7 & 97.7$\pm$2.2 & 0.16$\pm$0.08 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Mandible\_R & 95.7$\pm$2.5 & 0.17$\pm$0.08 & 92.8$\pm$2.3 & 0.45$\pm$0.06 & 91.3$\pm$1.1 & 0.36$\pm$0.10 & 95.6$\pm$2.6 & 0.13$\pm$0.09 & {\cellcolor[HTML]{F3F3F3}} & 91.5$\pm$2.4 & 0.47$\pm$0.07 & {\cellcolor[HTML]{F3F3F3}} & 97.7$\pm$2.6 & 0.14$\pm$0.09 & {\cellcolor[HTML]{F3F3F3}}
\\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise StructSeg19}
\end{table}

==> Tabs/tabs_ds5_pl/tab_pl_totalseg.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
Spleen & 97.6$\pm$15.6 & 1.95$\pm$0.40 & 97.2$\pm$6.4 & 0.37$\pm$0.36 & 96.6$\pm$3.2 & 0.36$\pm$0.44 & 97.1$\pm$6.8 & 1.65$\pm$0.39 & 99.7 & 97.8$\pm$6.9 & 0.29$\pm$0.41 & 99.5 & 97.2$\pm$6.8 & 1.67$\pm$0.40 & 99.5 \\
Kidney\_R & 95.9$\pm$16.9 & 0.19$\pm$0.73 & 94.3$\pm$6.8 & 1.23$\pm$0.73 & 95.7$\pm$4.7 & 0.29$\pm$0.30 & 96.1$\pm$7.1 & 0.21$\pm$0.76 & 99.7 & 94.9$\pm$7.1 & 1.07$\pm$0.76 & 99.7 & 97.1$\pm$7.2 & 0.21$\pm$0.78 & 99.7 \\
Kidney\_L & 96.1$\pm$26.7 & 1.15$\pm$6.45 & 93.7$\pm$6.8 & 1.61$\pm$0.71 & 91.9$\pm$17.5 & 1.72$\pm$8.64 & 97.2$\pm$6.9 & 1.00$\pm$0.72 &  & 94.2$\pm$6.9 & 1.46$\pm$0.72 & {} & 97.1$\pm$7.0 & 0.92$\pm$0.73 & {} \\
\rowcolor[HTML]{F3F3F3} 
GallBladder & 92.2$\pm$24.4 & 1.14$\pm$0.82 & 86.4$\pm$8.7 & 2.06$\pm$0.83 & 86.0$\pm$19.3 & 1.42$\pm$2.67 & 93.2$\pm$8.7 & 0.95$\pm$0.83 & 99.7 & 86.6$\pm$8.8 & 1.96$\pm$0.84 & 99.5 & 93.9$\pm$8.9 & 0.91$\pm$0.85 & 99.0 \\
Liver & 97.3$\pm$14.9 & 0.57$\pm$0.93 & 97.7$\pm$5.8 & 0.89$\pm$0.90 & 97.8$\pm$1.5 & 0.52$\pm$0.65 & 97.5$\pm$5.8 & 0.54$\pm$0.93 & 99.5 & 97.8$\pm$5.9 & 0.77$\pm$0.94 & 99.5 & 97.6$\pm$5.8 & 0.58$\pm$0.93 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
Stomach & 95.9$\pm$16.2 & 1.18$\pm$0.66 & 91.7$\pm$6.3 & 1.24$\pm$0.66 & 94.2$\pm$8.2 & 0.66$\pm$0.68 & 96.5$\pm$6.2 & 1.11$\pm$0.66 & 99.5 & 92.4$\pm$6.2 & 1.07$\pm$0.65 & 99.5 & 96.1$\pm$6.1 & 1.08$\pm$0.64 & 99.5 \\
Pancreas & 91.8$\pm$17.0 & 1.06$\pm$0.67 & 93.8$\pm$7.1 & 0.75$\pm$0.38 & 90.3$\pm$6.8 & 0.79$\pm$1.53 & 92.0$\pm$6.9 & 0.84$\pm$0.37 & 99.5 & 94.6$\pm$6.9 & 0.66$\pm$0.37 & 99.5 & 92.5$\pm$7.0 & 0.89$\pm$0.37 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Glnd\_Adrenal\_R & 83.0$\pm$13.5 & 0.55$\pm$1.17 & 90.3$\pm$13.1 & 0.28$\pm$0.38 & 87.8$\pm$11.2 & 0.50$\pm$1.60 & 84.2$\pm$13.3 & 0.43$\pm$0.39 & 94.0 & 90.6$\pm$13.1 & 0.22$\pm$0.38 & 98.0 & 85.2$\pm$13.5 & 0.43$\pm$0.41 & 98.0 \\
\rowcolor[HTML]{F3F3F3} 
Glnd\_Adrenal\_L & 84.2$\pm$12.2 & 1.03$\pm$0.36 & 87.9$\pm$12.5 & 0.42$\pm$0.38 & 85.4$\pm$13.5 & 0.31$\pm$0.26 & 84.8$\pm$12.5 & 0.87$\pm$0.39 &  & 88.3$\pm$12.5 & 0.40$\pm$0.39 & {\cellcolor[HTML]{F3F3F3}} & 85.0$\pm$12.6 & 0.93$\pm$0.39 & {\cellcolor[HTML]{F3F3F3}} \\
Lung\_LUL & 97.8$\pm$3.6 & 0.31$\pm$0.93 & 97.9$\pm$4.0 & 0.92$\pm$0.65 & 97.3$\pm$4.5 & 1.15$\pm$4.41 & 97.9$\pm$3.7 & 0.17$\pm$0.62 & 99.7 & 98.0$\pm$3.5 & 0.81$\pm$0.60 & 99.5 & 97.8$\pm$3.6 & 0.16$\pm$0.61 & 99.5 \\
Lung\_LLL & 96.5$\pm$24.0 & 0.21$\pm$0.98 & 97.8$\pm$2.2 & 0.59$\pm$0.48 & 95.7$\pm$8.5 & 0.72$\pm$1.68 & 96.5$\pm$2.1 & 0.21$\pm$0.47 &  & 97.8$\pm$2.3 & 0.54$\pm$0.49 & {} & 97.4$\pm$2.0 & 0.19$\pm$0.46 & {} \\
\rowcolor[HTML]{F3F3F3} 
Lung\_RUL & 97.5$\pm$20.5 & 0.30$\pm$1.48 & 95.8$\pm$2.6 & 0.91$\pm$0.94 & 92.0$\pm$19.5 & 0.77$\pm$1.37 & 97.7$\pm$2.5 & 0.20$\pm$0.98 & 99.5 & 96.4$\pm$2.3 & 0.73$\pm$0.97 & 99.5 & 97.8$\pm$2.6 & 0.21$\pm$1.00 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Lung\_RML & 92.0$\pm$6.2 & 0.47$\pm$1.41 & 97.7$\pm$3.3 & 0.71$\pm$1.39 & 94.8$\pm$6.5 & 0.83$\pm$1.31 & 92.3$\pm$3.3 & 0.22$\pm$1.50 &  & 98.1$\pm$3.3 & 0.66$\pm$1.40 & {\cellcolor[HTML]{F3F3F3}} & 93.1$\pm$3.3 & 0.23$\pm$1.37 & {\cellcolor[HTML]{F3F3F3}} \\
\rowcolor[HTML]{F3F3F3} 
Lung\_RLL & 97.4$\pm$26.8 & 0.16$\pm$2.45 & 95.5$\pm$3.8 & 0.65$\pm$1.16 & 97.2$\pm$5.9 & 0.43$\pm$0.83 & 97.2$\pm$3.6 & 0.21$\pm$1.19 &  & 95.9$\pm$3.5 & 0.63$\pm$1.17 & {\cellcolor[HTML]{F3F3F3}} & 97.0$\pm$3.7 & 0.21$\pm$1.10 & {\cellcolor[HTML]{F3F3F3}} \\
Eso & 94.8$\pm$2.9 & 0.61$\pm$0.15 & 84.7$\pm$11.8 & 0.79$\pm$4.56 & 94.1$\pm$2.1 & 0.24$\pm$0.24 & 94.4$\pm$3.1 & 0.45$\pm$0.16 & 99.7 & 85.4$\pm$3.0 & 0.64$\pm$0.15 & 98.0 & 94.5$\pm$3.1 & 0.46$\pm$0.16 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
Trachea & 96.7$\pm$5.8 & 0.36$\pm$0.12 & 92.8$\pm$2.7 & 0.93$\pm$1.98 & 96.0$\pm$5.0 & 0.27$\pm$0.47 & 97.1$\pm$6.1 & 0.27$\pm$0.12 & 99.5 & 92.9$\pm$6.1 & 0.86$\pm$0.12 & 99.7 & 97.2$\pm$6.0 & 0.27$\pm$0.11 & 99.7 \\
Glnd\_Thyroid & 91.7$\pm$14.7 & 0.41$\pm$0.96 & 82.2$\pm$4.7 & 1.15$\pm$0.28 & 90.2$\pm$9.2 & 0.37$\pm$0.45 & 92.6$\pm$14.5 & 0.28$\pm$0.96 & 99.7 & 82.7$\pm$14.5 & 0.95$\pm$0.96 & 94.0 & 93.3$\pm$14.6 & 0.26$\pm$0.97 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
SmallBowel & 91.2$\pm$26.4 & 1.63$\pm$2.53 & 90.5$\pm$16.6 & 2.39$\pm$2.42 & 87.4$\pm$14.0 & 1.56$\pm$1.77 & 91.2$\pm$16.6 & 1.55$\pm$2.62 & 99.7 & 91.2$\pm$16.4 & 2.22$\pm$2.54 & 99.5 & 91.1$\pm$16.6 & 1.52$\pm$2.41 & 99.5 \\
Duodenum & 87.3$\pm$26.0 & 1.87$\pm$1.26 & 82.3$\pm$16.1 & 2.43$\pm$1.18 & 82.9$\pm$18.3 & 1.02$\pm$1.08 & 88.8$\pm$16.1 & 1.81$\pm$1.26 & 99.5 & 82.9$\pm$16.0 & 2.29$\pm$1.18 & 99.5 & 89.4$\pm$15.9 & 1.74$\pm$1.19 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Colon & 90.2$\pm$16.0 & 2.54$\pm$1.21 & 92.3$\pm$15.9 & 2.88$\pm$1.15 & 89.9$\pm$7.9 & 1.55$\pm$1.90 & 90.4$\pm$15.8 & 2.36$\pm$1.23 & 99.5 & 92.9$\pm$15.9 & 2.72$\pm$1.13 & 99.5 & 90.7$\pm$15.7 & 2.49$\pm$1.13 & 99.7 \\
UrinaryBladder & 89.1$\pm$9.5 & 2.98$\pm$1.08 & 93.3$\pm$9.3 & 1.93$\pm$0.99 & 92.5$\pm$7.6 & 1.27$\pm$1.97 & 89.2$\pm$9.6 & 2.85$\pm$1.03 & 99.5 & 93.6$\pm$9.7 & 1.82$\pm$0.94 & 98.0 & 89.7$\pm$9.5 & 2.99$\pm$0.96 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Prostate & 81.7$\pm$38.0 & 0.52$\pm$2.06 & 85.2$\pm$18.2 & 3.82$\pm$1.29 & 72.8$\pm$33.5 & 1.45$\pm$1.72 & 83.3$\pm$17.9 & 0.35$\pm$1.47 & 99.5 & 85.5$\pm$17.7 & 3.62$\pm$1.36 & 96.0 & 83.8$\pm$17.9 & 0.33$\pm$1.44 & 99.5
 \\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise TotalSegmentator -- `Organ' subgroup}
\end{table}



\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
Heart & 95.2$\pm$14.7 & 0.42$\pm$0.20 & 97.0$\pm$1.9 & 1.67$\pm$0.22 & 95.9$\pm$1.4 & 1.10$\pm$3.24 & 94.9$\pm$14.7 & 0.43$\pm$0.18 & 99.7 & 97.1$\pm$14.7 & 1.64$\pm$0.19 & 99.0 & 94.8$\pm$14.8 & 0.46$\pm$0.20 & 99.5 \\
A\_Aorta & 96.0$\pm$16.7 & 0.44$\pm$0.95 & 94.3$\pm$2.9 & 0.75$\pm$0.54 & 96.7$\pm$4.7 & 0.30$\pm$0.57 & 96.5$\pm$16.7 & 0.41$\pm$0.85 & 99.7 & 95.0$\pm$16.9 & 0.75$\pm$0.86 & 99.0 & 96.0$\pm$16.8 & 0.42$\pm$0.86 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
V\_Pulmonary & 89.8$\pm$15.5 & 0.47$\pm$0.14 & 75.0$\pm$6.4 & 1.39$\pm$1.04 & 93.1$\pm$3.1 & 0.23$\pm$0.13 & 91.3$\pm$15.5 & 0.31$\pm$0.16 & 99.0 & 75.5$\pm$15.3 & 1.37$\pm$0.14 & 99.0 & 90.7$\pm$15.4 & 0.30$\pm$0.14 & 99.0 \\
A\_BrachiocephalicTrunk & 89.8$\pm$16.2 & 0.32$\pm$0.43 & 89.8$\pm$16.2 & 0.32$\pm$0.43 & 93.8$\pm$3.0 & 0.22$\pm$0.18 & 90.8$\pm$16.3 & 0.22$\pm$0.44 & 99.0 & 97.3$\pm$16.1 & 0.72$\pm$0.42 & 99.0 & 90.5$\pm$16.3 & 0.22$\pm$0.44 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
A\_Subclavian\_L & 94.6$\pm$3.5 & 0.44$\pm$0.28 & 82.1$\pm$8.5 & 2.80$\pm$25.60 & 91.6$\pm$3.5 & 0.33$\pm$0.47 & 94.9$\pm$3.6 & 0.27$\pm$0.29 & 99.7 & 82.4$\pm$3.5 & 2.69$\pm$0.28 & 94.0 & 95.3$\pm$3.6 & 0.27$\pm$0.29 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
A\_Subclavian\_R & 94.1$\pm$3.3 & 0.23$\pm$0.17 & 84.9$\pm$6.0 & 1.61$\pm$6.51 & 91.5$\pm$3.4 & 0.22$\pm$0.15 & 93.3$\pm$3.4 & 0.17$\pm$0.18 & {\cellcolor[HTML]{F3F3F3}} & 85.5$\pm$3.3 & 1.45$\pm$0.16 & {\cellcolor[HTML]{F3F3F3}} & 93.0$\pm$3.3 & 0.17$\pm$0.17 & {\cellcolor[HTML]{F3F3F3}} \\
A\_CommonCarotid\_L & 91.2$\pm$5.4 & 0.35$\pm$0.28 & 89.0$\pm$7.4 & 1.13$\pm$3.61 & 90.3$\pm$4.8 & 0.23$\pm$0.22 & 91.1$\pm$5.4 & 0.24$\pm$0.28 & 99.5 & 89.7$\pm$5.2 & 1.04$\pm$0.26 & 99.7 & 90.6$\pm$5.5 & 0.23$\pm$0.29 & 99.5 \\
A\_CommonCarotid\_R & 96.6$\pm$3.3 & 0.28$\pm$0.99 & 85.7$\pm$9.8 & 0.69$\pm$3.32 & 93.2$\pm$2.4 & 0.15$\pm$0.13 & 97.4$\pm$3.3 & 0.26$\pm$1.02 & {} & 86.6$\pm$3.3 & 0.61$\pm$1.00 & {} & 97.2$\pm$3.5 & 0.26$\pm$1.01 & {} \\
\rowcolor[HTML]{F3F3F3} 
V\_Brachiocephalic\_L & 90.4$\pm$26.2 & 0.37$\pm$1.97 & 91.2$\pm$4.9 & 0.43$\pm$0.12 & 91.5$\pm$15.7 & 0.44$\pm$1.59 & 91.2$\pm$16.1 & 0.31$\pm$2.11 & 99.5 & 92.2$\pm$16.2 & 0.34$\pm$1.90 & 99.5 & 92.2$\pm$16.2 & 0.33$\pm$1.91 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
V\_Brachiocephalic\_R & 88.7$\pm$15.0 & 0.32$\pm$0.81 & 89.9$\pm$6.0 & 0.78$\pm$0.29 & 89.8$\pm$11.4 & 0.37$\pm$0.57 & 89.1$\pm$15.3 & 0.24$\pm$0.84 & {\cellcolor[HTML]{F3F3F3}} & 90.6$\pm$15.4 & 0.65$\pm$0.84 & {\cellcolor[HTML]{F3F3F3}} & 90.0$\pm$15.3 & 0.24$\pm$0.83 & {\cellcolor[HTML]{F3F3F3}} \\
LLA & 92.6$\pm$3.4 & 0.46$\pm$0.15 & 92.3$\pm$3.6 & 0.99$\pm$0.17 & 93.2$\pm$2.7 & 0.20$\pm$0.11 & 91.7$\pm$3.3 & 0.16$\pm$0.15 & 99.5 & 92.9$\pm$3.5 & 0.90$\pm$0.17 & 99.7 & 92.5$\pm$3.4 & 0.18$\pm$0.16 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
V\_VenaCava\_S & 93.8$\pm$21.4 & 0.23$\pm$2.35 & 92.0$\pm$4.3 & 1.02$\pm$0.25 & 88.4$\pm$24.2 & 0.42$\pm$0.83 & 93.7$\pm$21.4 & 0.18$\pm$2.44 & 99.5 & 92.0$\pm$21.4 & 0.83$\pm$2.23 & 99.0 & 93.7$\pm$21.5 & 0.17$\pm$2.23 & 99.5 \\
V\_VenaCava\_I & 93.9$\pm$9.8 & 1.03$\pm$1.05 & 83.6$\pm$7.6 & 1.74$\pm$0.48 & 92.3$\pm$6.3 & 0.47$\pm$0.38 & 95.2$\pm$9.8 & 0.77$\pm$1.00 & 99.5 & 84.5$\pm$9.7 & 1.72$\pm$0.99 & 99.0 & 95.8$\pm$9.7 & 0.77$\pm$0.99 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
V\_Portal\_Splenic & 85.5$\pm$29.3 & 1.29$\pm$0.62 & 85.5$\pm$29.3 & 1.29$\pm$0.62 & 85.1$\pm$12.1 & 0.67$\pm$0.72 & 86.7$\pm$29.1 & 1.12$\pm$0.63 & 99.0 & 89.0$\pm$29.1 & 0.32$\pm$0.62 & 98.0 & 86.0$\pm$29.1 & 1.18$\pm$0.63 & 98.0 \\
A\_Iliac\_L & 94.4$\pm$3.1 & 0.61$\pm$0.19 & 94.4$\pm$3.1 & 0.61$\pm$0.19 & 93.2$\pm$3.0 & 0.25$\pm$0.38 & 95.1$\pm$3.3 & 0.50$\pm$0.20 & 99.5 & 91.1$\pm$3.5 & 0.45$\pm$0.22 & 99.0 & 96.0$\pm$3.3 & 0.50$\pm$0.20 & 99.7 \\
A\_Iliac\_R & 91.9$\pm$19.5 & 0.45$\pm$0.15 & 91.9$\pm$19.5 & 0.45$\pm$0.15 & 93.5$\pm$3.8 & 0.19$\pm$0.26 & 91.9$\pm$19.6 & 0.39$\pm$0.18 & {} & 90.6$\pm$19.8 & 0.36$\pm$0.20 & {} & 91.1$\pm$19.7 & 0.36$\pm$0.19 & {} \\
\rowcolor[HTML]{F3F3F3} 
V\_Iliac\_L & 92.2$\pm$3.0 & 0.48$\pm$0.13 & 92.2$\pm$3.0 & 0.48$\pm$0.13 & 94.1$\pm$2.8 & 0.18$\pm$0.10 & 92.9$\pm$3.3 & 0.43$\pm$0.15 & 99.0 & 92.6$\pm$3.5 & 0.31$\pm$0.17 & 99.7 & 92.6$\pm$3.3 & 0.45$\pm$0.15 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
V\_Iliac\_R & 94.2$\pm$4.9 & 0.44$\pm$0.31 & 94.2$\pm$4.9 & 0.44$\pm$0.31 & 92.9$\pm$5.6 & 0.22$\pm$0.20 & 93.6$\pm$4.8 & 0.45$\pm$0.27 & {\cellcolor[HTML]{F3F3F3}} & 91.9$\pm$4.9 & 0.33$\pm$0.28 & {\cellcolor[HTML]{F3F3F3}} & 94.4$\pm$4.9 & 0.47$\pm$0.28 & {\cellcolor[HTML]{F3F3F3}}
 \\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise TotalSegmentator -- `Cardiac' subgroup}
\end{table}




\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
Bone\_Humerus\_L & 96.9$\pm$17.5 & 2.84$\pm$0.20 & 96.9$\pm$17.5 & 2.84$\pm$0.20 & 93.5$\pm$7.1 & 0.57$\pm$0.97 & 97.1$\pm$17.6 & 2.77$\pm$0.21 & 99.5 & 97.0$\pm$17.5 & 0.69$\pm$0.20 & 99.7 & 97.3$\pm$17.4 & 2.97$\pm$0.19 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Humerus\_R & 96.6$\pm$17.3 & 4.31$\pm$0.17 & 96.6$\pm$17.3 & 4.31$\pm$0.17 & 96.5$\pm$2.0 & 5.20$\pm$12.27 & 97.1$\pm$17.0 & 3.88$\pm$0.17 & {\cellcolor[HTML]{F3F3F3}} & 93.7$\pm$17.0 & 0.39$\pm$0.17 & {\cellcolor[HTML]{F3F3F3}} & 97.2$\pm$17.0 & 4.19$\pm$0.17 & {\cellcolor[HTML]{F3F3F3}} \\
Bone\_Scapula\_L & 94.1$\pm$21.1 & 1.16$\pm$0.18 & 94.1$\pm$21.1 & 1.16$\pm$0.18 & 94.8$\pm$1.9 & 0.49$\pm$1.16 & 93.8$\pm$21.4 & 0.97$\pm$0.17 & 99.5 & 94.5$\pm$21.2 & 0.20$\pm$0.16 & 99.0 & 94.0$\pm$21.5 & 0.98$\pm$0.19 & 99.5 \\
Bone\_Scapula\_R & 95.1$\pm$1.7 & 1.95$\pm$0.07 & 95.1$\pm$1.7 & 1.95$\pm$0.07 & 95.2$\pm$2.1 & 0.35$\pm$0.59 & 94.4$\pm$1.9 & 1.63$\pm$0.08 & {} & 92.6$\pm$2.0 & 0.45$\pm$0.09 & {} & 93.9$\pm$2.1 & 1.48$\pm$0.10 & {} \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Clavicula\_L & 94.5$\pm$0.8 & 0.60$\pm$0.10 & 94.5$\pm$0.8 & 0.60$\pm$0.10 & 96.6$\pm$1.8 & 1.76$\pm$7.40 & 95.2$\pm$0.9 & 0.45$\pm$0.11 & 99.5 & 94.2$\pm$0.9 & 0.36$\pm$0.11 & 99.7 & 96.0$\pm$1.0 & 0.46$\pm$0.13 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Clavicula\_R & 98.4$\pm$16.1 & 1.52$\pm$0.19 & 98.4$\pm$16.1 & 1.52$\pm$0.19 & 95.5$\pm$3.2 & 1.72$\pm$9.22 & 98.3$\pm$16.0 & 1.37$\pm$0.20 & {\cellcolor[HTML]{F3F3F3}} & 96.6$\pm$16.1 & 0.52$\pm$0.22 & {\cellcolor[HTML]{F3F3F3}} & 98.4$\pm$15.8 & 1.29$\pm$0.18 & {\cellcolor[HTML]{F3F3F3}} \\
Bone\_Femur\_L & 97.4$\pm$15.4 & 3.51$\pm$0.29 & 97.4$\pm$15.4 & 3.51$\pm$0.29 & 94.6$\pm$14.3 & 9.92$\pm$40.53 & 97.5$\pm$0.7 & 3.28$\pm$0.11 & 99.7 & 92.0$\pm$0.6 & 5.77$\pm$0.10 & 99.5 & 97.6$\pm$0.7 & 3.06$\pm$0.11 & 99.5 \\
Bone\_Femur\_R & 95.8$\pm$0.5 & 6.85$\pm$0.08 & 95.8$\pm$0.5 & 6.85$\pm$0.08 & 98.4$\pm$0.4 & 0.52$\pm$1.08 & 96.3$\pm$0.2 & 6.26$\pm$0.06 & {} & 94.6$\pm$0.2 & 5.95$\pm$0.06 & {} & 96.9$\pm$0.3 & 5.96$\pm$0.07 & {} \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Hip\_L & 96.6$\pm$1.6 & 0.32$\pm$1.13 & 96.6$\pm$1.6 & 0.32$\pm$1.13 & 97.3$\pm$1.5 & 0.44$\pm$0.89 & 97.0$\pm$1.9 & 0.29$\pm$0.14 & 99.5 & 98.2$\pm$2.0 & 0.27$\pm$0.15 & 99.5 & 97.1$\pm$2.0 & 0.31$\pm$0.14 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Hip\_R & 95.9$\pm$31.6 & 0.34$\pm$0.10 & 95.9$\pm$31.6 & 0.34$\pm$0.10 & 98.0$\pm$0.3 & 0.20$\pm$0.45 & 97.0$\pm$31.9 & 0.27$\pm$0.11 & {\cellcolor[HTML]{F3F3F3}} & 97.7$\pm$32.0 & 0.37$\pm$0.11 & {\cellcolor[HTML]{F3F3F3}} & 96.5$\pm$31.8 & 0.30$\pm$0.10 & {\cellcolor[HTML]{F3F3F3}} \\
SpinalCord & 92.7$\pm$16.8 & 0.27$\pm$0.24 & 93.4$\pm$3.0 & 0.88$\pm$0.24 & 94.5$\pm$3.7 & 0.20$\pm$0.13 & 92.7$\pm$16.5 & 0.26$\pm$0.24 & 99.5 & 94.1$\pm$16.7 & 0.84$\pm$0.26 & 99.7 & 93.1$\pm$16.4 & 0.27$\pm$0.23 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Musc\_GluteusMax\_L & 98.9$\pm$5.2 & 0.84$\pm$1.41 & 98.9$\pm$5.2 & 0.84$\pm$1.41 & 93.8$\pm$7.7 & 3.56$\pm$10.31 & 98.7$\pm$5.4 & 0.76$\pm$1.50 & 99.5 & 96.7$\pm$5.4 & 0.58$\pm$1.43 & 99.5 & 98.8$\pm$5.5 & 0.75$\pm$1.45 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
Musc\_GluteusMax\_R & 98.1$\pm$2.0 & 0.93$\pm$0.34 & 98.1$\pm$2.0 & 0.93$\pm$0.34 & 95.2$\pm$4.0 & 2.29$\pm$4.92 & 97.9$\pm$2.2 & 0.71$\pm$0.34 & {\cellcolor[HTML]{F3F3F3}} & 97.5$\pm$2.1 & 0.54$\pm$0.34 & {\cellcolor[HTML]{F3F3F3}} & 97.7$\pm$2.3 & 0.66$\pm$0.35 & {\cellcolor[HTML]{F3F3F3}} \\
Musc\_GluteusMed\_L & 98.2$\pm$1.5 & 0.43$\pm$0.22 & 98.2$\pm$1.5 & 0.43$\pm$0.22 & 94.0$\pm$3.0 & 0.93$\pm$1.57 & 98.4$\pm$1.5 & 0.45$\pm$0.23 & 99.7 & 97.5$\pm$1.6 & 0.30$\pm$0.24 & 99.5 & 98.3$\pm$1.5 & 0.47$\pm$0.23 & 99.5 \\
Musc\_GluteusMed\_R & 97.6$\pm$7.3 & 0.74$\pm$0.22 & 97.6$\pm$7.3 & 0.74$\pm$0.22 & 93.7$\pm$3.8 & 0.76$\pm$0.73 & 97.3$\pm$7.5 & 0.47$\pm$0.21 & {} & 97.0$\pm$7.7 & 0.37$\pm$0.22 & {} & 97.5$\pm$7.4 & 0.50$\pm$0.19 & {} \\
\rowcolor[HTML]{F3F3F3} 
Musc\_GluteusMin\_L & 97.1$\pm$2.3 & 0.56$\pm$0.16 & 97.1$\pm$2.3 & 0.56$\pm$0.16 & 91.9$\pm$3.0 & 0.93$\pm$1.75 & 97.3$\pm$2.2 & 0.42$\pm$0.16 & 99.7 & 95.6$\pm$2.4 & 0.42$\pm$0.17 & 99.5 & 97.4$\pm$2.1 & 0.43$\pm$0.15 & 99.7 \\
\rowcolor[HTML]{F3F3F3} 
Musc\_GluteusMin\_R & 98.0$\pm$1.1 & 0.39$\pm$0.08 & 98.0$\pm$1.1 & 0.39$\pm$0.08 & 93.0$\pm$1.7 & 0.41$\pm$0.16 & 98.2$\pm$1.1 & 0.36$\pm$0.10 & {\cellcolor[HTML]{F3F3F3}} & 93.6$\pm$1.0 & 0.29$\pm$0.08 & {\cellcolor[HTML]{F3F3F3}} & 98.3$\pm$1.0 & 0.34$\pm$0.09 & {\cellcolor[HTML]{F3F3F3}} \\
Musc\_Autochthon\_L & 94.2$\pm$0.8 & 0.37$\pm$0.11 & 94.2$\pm$0.8 & 0.37$\pm$0.11 & 95.8$\pm$1.3 & 0.38$\pm$0.15 & 93.9$\pm$0.9 & 0.32$\pm$0.12 & 99.7 & 96.9$\pm$0.7 & 2.06$\pm$0.10 & 99.0 & 94.3$\pm$1.1 & 0.29$\pm$0.14 & 99.0 \\
Musc\_Autochthon\_R & 94.6$\pm$0.8 & 0.41$\pm$0.12 & 94.6$\pm$0.8 & 0.41$\pm$0.12 & 95.8$\pm$1.2 & 0.37$\pm$0.12 & 94.8$\pm$0.8 & 0.41$\pm$0.11 & {} & 97.5$\pm$0.7 & 2.09$\pm$0.10 & {} & 95.1$\pm$0.9 & 0.39$\pm$0.12 & {} \\
\rowcolor[HTML]{F3F3F3} 
Musc\_Iliopsoas\_L & 94.3$\pm$19.7 & 0.37$\pm$0.18 & 94.3$\pm$19.7 & 0.37$\pm$0.18 & 90.3$\pm$9.0 & 0.50$\pm$0.86 & 93.5$\pm$19.6 & 0.36$\pm$0.19 & 99.5 & 93.7$\pm$19.7 & 0.22$\pm$0.20 & 99.0 & 92.5$\pm$19.8 & 0.33$\pm$0.20 & 99.0 \\
\rowcolor[HTML]{F3F3F3} 
Musc\_Iliopsoas\_R & 95.0$\pm$9.1 & 0.39$\pm$0.27 & 95.0$\pm$9.1 & 0.39$\pm$0.27 & 90.0$\pm$9.5 & 0.44$\pm$0.57 & 94.9$\pm$9.1 & 0.32$\pm$0.25 & {\cellcolor[HTML]{F3F3F3}} & 93.9$\pm$9.2 & 0.31$\pm$0.26 & {\cellcolor[HTML]{F3F3F3}} & 95.6$\pm$9.2 & 0.30$\pm$0.26 & {\cellcolor[HTML]{F3F3F3}} \\
Brain & 97.9$\pm$36.4 & 0.56$\pm$1.01 & 97.9$\pm$36.4 & 0.56$\pm$1.01 & 88.3$\pm$28.0 & 7.85$\pm$24.00 & 98.2$\pm$16.3 & 0.51$\pm$1.07 & 99.5 & 97.7$\pm$16.3 & 0.28$\pm$1.01 & 99.5 & 98.2$\pm$16.4 & 0.51$\pm$1.04 & 99.5 \\
\rowcolor[HTML]{F3F3F3} 
Skull & 93.1$\pm$35.4 & 3.91$\pm$0.20 & 93.1$\pm$35.4 & 3.91$\pm$0.20 & 89.5$\pm$21.0 & 1.07$\pm$2.79 & 92.5$\pm$35.4 & 3.66$\pm$0.21 & 99.7 & 81.3$\pm$35.5 & 1.47$\pm$0.22 & 99.0 & 92.0$\pm$35.5 & 3.45$\pm$0.21 & 99.5

 \\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise TotalSegmentator -- `Muscles' subgroup}
\end{table}




\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib1\_L & 93.6$\pm$3.3 & 0.16$\pm$0.23 & 93.6$\pm$3.3 & 0.16$\pm$0.23 & 92.4$\pm$8.9 & 0.15$\pm$0.13 & 93.3$\pm$3.3 & 0.14$\pm$0.21 & {\cellcolor[HTML]{F3F3F3}96.0} & 91.0$\pm$3.1 & 0.79$\pm$0.19 & {\cellcolor[HTML]{F3F3F3}96.0} & 92.4$\pm$3.1 & 0.14$\pm$0.19 & {\cellcolor[HTML]{F3F3F3}98.0} \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib2\_L & 89.9$\pm$1.7 & 0.95$\pm$0.95 & 89.9$\pm$1.7 & 0.95$\pm$0.95 & 95.4$\pm$1.5 & 0.19$\pm$0.76 & 90.2$\pm$1.5 & 0.74$\pm$1.02 &  & 91.0$\pm$1.6 & 0.63$\pm$0.99 &  & 89.5$\pm$1.6 & 0.69$\pm$0.92 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib3\_L & 94.7$\pm$17.0 & 0.91$\pm$1.06 & 94.7$\pm$17.0 & 0.91$\pm$1.06 & 94.9$\pm$3.0 & 0.13$\pm$0.20 & 94.9$\pm$17.0 & 0.85$\pm$1.08 &  & 88.3$\pm$17.1 & 1.40$\pm$0.99 &  & 94.5$\pm$17.0 & 0.90$\pm$1.04 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib4\_L & 94.5$\pm$18.9 & 0.76$\pm$1.82 & 94.5$\pm$18.9 & 0.76$\pm$1.82 & 94.9$\pm$3.8 & 0.20$\pm$0.48 & 93.9$\pm$18.7 & 0.63$\pm$1.77 &  & 87.6$\pm$18.8 & 1.94$\pm$1.66 &  & 94.1$\pm$18.8 & 0.61$\pm$1.67 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib5\_L & 94.2$\pm$29.7 & 1.52$\pm$4.61 & 94.2$\pm$29.7 & 1.52$\pm$4.61 & 91.5$\pm$15.6 & 0.42$\pm$1.23 & 94.3$\pm$29.6 & 1.06$\pm$4.53 &  & 87.4$\pm$29.8 & 2.07$\pm$4.20 &  & 93.4$\pm$29.4 & 1.11$\pm$4.29 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib6\_L & 93.2$\pm$23.9 & 1.64$\pm$3.32 & 93.2$\pm$23.9 & 1.64$\pm$3.32 & 93.0$\pm$11.4 & 0.37$\pm$0.97 & 92.8$\pm$24.1 & 1.51$\pm$3.35 &  & 89.9$\pm$24.3 & 1.70$\pm$3.29 &  & 92.8$\pm$24.3 & 1.55$\pm$3.15 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib7\_L & 94.5$\pm$20.7 & 2.71$\pm$4.08 & 94.5$\pm$20.7 & 2.71$\pm$4.08 & 93.9$\pm$5.4 & 0.33$\pm$0.50 & 95.8$\pm$20.8 & 2.36$\pm$4.01 &  & 90.9$\pm$20.7 & 1.51$\pm$3.94 &  & 95.6$\pm$20.8 & 2.25$\pm$3.69 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib8\_L & 94.6$\pm$21.1 & 4.29$\pm$4.00 & 94.6$\pm$21.1 & 4.29$\pm$4.00 & 90.4$\pm$15.0 & 0.89$\pm$2.41 & 95.2$\pm$21.1 & 4.15$\pm$4.04 &  & 90.8$\pm$20.9 & 1.38$\pm$3.75 &  & 95.5$\pm$20.9 & 3.82$\pm$3.80 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib9\_L & 94.0$\pm$19.4 & 2.83$\pm$5.21 & 94.0$\pm$19.4 & 2.83$\pm$5.21 & 89.9$\pm$16.2 & 1.32$\pm$3.61 & 94.5$\pm$19.3 & 2.74$\pm$4.83 &  & 90.4$\pm$19.5 & 0.99$\pm$4.55 &  & 95.0$\pm$19.5 & 2.57$\pm$4.40 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib10\_L & 93.0$\pm$22.9 & 1.51$\pm$6.63 & 93.0$\pm$22.9 & 1.51$\pm$6.63 & 87.5$\pm$23.7 & 2.24$\pm$5.96 & 91.9$\pm$13.2 & 1.48$\pm$6.45 &  & 91.3$\pm$13.2 & 0.13$\pm$6.14 &  & 91.5$\pm$13.1 & 1.46$\pm$6.42 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib11\_L & 93.0$\pm$22.4 & 0.36$\pm$8.01 & 93.0$\pm$22.4 & 0.36$\pm$8.01 & 87.5$\pm$23.4 & 2.55$\pm$7.91 & 92.1$\pm$12.1 & 0.34$\pm$8.12 &  & 93.1$\pm$12.2 & 0.30$\pm$8.02 &  & 92.7$\pm$12.1 & 0.32$\pm$7.51 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib12\_L & 94.2$\pm$26.2 & 0.54$\pm$0.41 & 94.2$\pm$26.2 & 0.54$\pm$0.41 & 91.5$\pm$8.3 & 1.02$\pm$4.36 & 94.7$\pm$16.3 & 0.33$\pm$0.41 &  & 93.3$\pm$16.1 & 0.20$\pm$0.39 &  & 94.5$\pm$16.3 & 0.31$\pm$0.40 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib1\_R & 91.2$\pm$5.6 & 0.11$\pm$0.17 & 91.2$\pm$5.6 & 0.11$\pm$0.17 & 94.0$\pm$2.6 & 0.15$\pm$0.17 & 91.8$\pm$5.6 & 0.14$\pm$0.15 &  & 91.3$\pm$5.6 & 0.71$\pm$0.15 &  & 91.9$\pm$5.5 & 0.15$\pm$0.14 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib2\_R & 94.5$\pm$3.5 & 0.23$\pm$0.94 & 94.5$\pm$3.5 & 0.23$\pm$0.94 & 95.1$\pm$3.4 & 0.14$\pm$0.41 & 94.6$\pm$3.4 & 0.09$\pm$0.91 &  & 91.0$\pm$3.2 & 0.59$\pm$0.89 &  & 94.7$\pm$3.2 & 0.09$\pm$0.89 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib3\_R & 92.8$\pm$9.1 & 0.48$\pm$0.75 & 92.8$\pm$9.1 & 0.48$\pm$0.75 & 93.7$\pm$5.8 & 0.20$\pm$0.38 & 93.7$\pm$9.1 & 0.34$\pm$1.14 &  & 91.6$\pm$9.0 & 0.77$\pm$1.05 &  & 93.9$\pm$9.3 & 0.38$\pm$1.11 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib4\_R & 90.5$\pm$18.8 & 0.83$\pm$2.02 & 90.5$\pm$18.8 & 0.83$\pm$2.02 & 94.4$\pm$7.4 & 0.10$\pm$0.10 & 90.4$\pm$18.6 & 0.73$\pm$1.92 &  & 91.6$\pm$18.5 & 0.31$\pm$1.86 &  & 91.1$\pm$18.4 & 0.73$\pm$1.85 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib5\_R & 90.3$\pm$26.5 & 1.70$\pm$2.42 & 90.3$\pm$26.5 & 1.70$\pm$2.42 & 89.7$\pm$20.6 & 0.72$\pm$2.36 & 90.7$\pm$16.4 & 1.49$\pm$2.51 &  & 90.4$\pm$16.3 & 1.02$\pm$2.43 &  & 91.4$\pm$16.5 & 1.43$\pm$2.31 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib6\_R & 93.4$\pm$18.9 & 1.52$\pm$2.45 & 93.4$\pm$18.9 & 1.52$\pm$2.45 & 89.6$\pm$18.0 & 1.05$\pm$3.01 & 93.4$\pm$13.0 & 1.38$\pm$2.54 &  & 90.0$\pm$13.1 & 1.56$\pm$2.36 &  & 93.0$\pm$13.1 & 1.46$\pm$2.45 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib7\_R & 94.2$\pm$21.0 & 1.56$\pm$3.51 & 94.2$\pm$21.0 & 1.56$\pm$3.51 & 90.7$\pm$16.5 & 0.77$\pm$1.61 & 95.5$\pm$21.3 & 1.57$\pm$3.36 &  & 88.8$\pm$21.4 & 1.94$\pm$3.35 &  & 94.6$\pm$21.3 & 1.62$\pm$3.08 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib8\_R & 95.5$\pm$18.3 & 1.88$\pm$4.08 & 95.5$\pm$18.3 & 1.88$\pm$4.08 & 91.8$\pm$10.0 & 0.81$\pm$1.83 & 95.0$\pm$18.0 & 1.78$\pm$4.22 &  & 90.5$\pm$17.9 & 1.20$\pm$4.07 &  & 95.5$\pm$17.9 & 1.67$\pm$4.06 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib9\_R & 95.9$\pm$21.4 & 2.48$\pm$5.16 & 95.9$\pm$21.4 & 2.48$\pm$5.16 & 91.7$\pm$11.6 & 1.21$\pm$2.97 & 96.3$\pm$21.6 & 2.25$\pm$3.18 &  & 90.8$\pm$21.8 & 1.54$\pm$3.04 &  & 95.5$\pm$21.7 & 2.05$\pm$3.06 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib10\_R & 96.3$\pm$23.3 & 2.50$\pm$7.23 & 96.3$\pm$23.3 & 2.50$\pm$7.23 & 90.6$\pm$18.4 & 1.33$\pm$4.17 & 95.9$\pm$23.3 & 2.30$\pm$7.41 &  & 91.7$\pm$23.4 & 2.48$\pm$6.90 &  & 95.9$\pm$23.4 & 2.27$\pm$7.24 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib11\_R & 96.4$\pm$22.8 & 1.85$\pm$6.95 & 96.4$\pm$22.8 & 1.85$\pm$6.95 & 90.4$\pm$18.2 & 1.50$\pm$5.23 & 97.5$\pm$22.7 & 1.71$\pm$6.70 &  & 90.6$\pm$22.7 & 1.30$\pm$6.07 &  & 97.6$\pm$22.9 & 1.60$\pm$6.06 &  \\
\rowcolor[HTML]{F3F3F3} 
Bone\_Rib12\_R & 97.1$\pm$27.5 & 0.63$\pm$0.07 & 97.1$\pm$27.5 & 0.63$\pm$0.07 & 89.5$\pm$13.9 & 1.32$\pm$3.03 & 97.4$\pm$27.5 & 0.46$\pm$0.10 &  & 90.8$\pm$27.6 & 0.57$\pm$0.12 &  & 97.2$\pm$27.6 & 0.41$\pm$0.12 &  \\
Bone\_Sternum & 94.1$\pm$5.8 & 0.63$\pm$0.55 & 94.1$\pm$5.8 & 0.63$\pm$0.55 & 94.9$\pm$2.7 & 0.36$\pm$0.91 & 95.5$\pm$5.7 & 0.35$\pm$0.55 & {99.7} & 91.8$\pm$5.5 & 1.13$\pm$0.53 & {99.5} & 94.7$\pm$5.5 & 0.36$\pm$0.53 & {99.7} \\
\rowcolor[HTML]{F3F3F3} 
Bone\_CostalCartilages & 88.7$\pm$5.0 & 0.18$\pm$0.74 & 88.7$\pm$5.0 & 0.18$\pm$0.74 & 91.2$\pm$3.2 & 0.44$\pm$0.59 & 88.6$\pm$5.0 & 0.16$\pm$0.74 & {\cellcolor[HTML]{F3F3F3}99.5} & 91.0$\pm$5.1 & 1.13$\pm$0.75 & {\cellcolor[HTML]{F3F3F3}99.7} & 88.0$\pm$5.0 & 0.16$\pm$0.75 & {\cellcolor[HTML]{F3F3F3}99.5}

 \\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise TotalSegmentator -- `Ribs' subgroup}
\end{table}




\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|ll|ll|ll|ll|r|ll|r|ll|r|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{nnUNet} & \multicolumn{2}{c|}{nnUNet$^{E_{36}}$} & \multicolumn{2}{c|}{MultiTalent} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{5}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}$} & \multicolumn{3}{c|}{SUNSeg$^{\mathcal{U}_{36}}_{\text{ft}}$} \\ \cline{2-16} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{}} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & \multicolumn{1}{l|}{ASD$\downarrow$} & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } & DSC$\uparrow$ & ASD$\downarrow$ & \multicolumn{1}{r|}{$\mathcal{T}$$\uparrow$ } \\ \hline
\rowcolor[HTML]{F3F3F3} 
Bone\_Sacrum & 93.4$\pm$1.8 & 0.25$\pm$0.13 & 93.4$\pm$1.8 & 0.25$\pm$0.13 & 95.0$\pm$2.2 & 0.48$\pm$0.27 & 93.9$\pm$1.9 & 0.19$\pm$0.14 & {\cellcolor[HTML]{F3F3F3}99.0} & 97.3$\pm$1.9 & 0.26$\pm$0.14 & {\cellcolor[HTML]{F3F3F3}99.5} & 93.8$\pm$2.1 & 0.20$\pm$0.16 & {\cellcolor[HTML]{F3F3F3}99.5} \\
Bone\_Vert\_C1 & 94.5$\pm$20.3 & 0.25$\pm$0.53 & 94.5$\pm$20.3 & 0.25$\pm$0.53 & 94.3$\pm$4.2 & 0.42$\pm$0.53 & 95.3$\pm$10.2 & 0.23$\pm$0.50 & {96.0} & 86.9$\pm$10.4 & 0.27$\pm$0.52 &  & 94.6$\pm$10.0 & 0.24$\pm$0.49 & {96.0} \\
Bone\_Vert\_C2 & 98.0$\pm$20.7 & 0.31$\pm$3.04 & 98.0$\pm$20.7 & 0.31$\pm$3.04 & 93.2$\pm$20.1 & 0.09$\pm$0.08 & 97.9$\pm$10.5 & 0.14$\pm$0.47 &  & 95.7$\pm$10.5 & 0.18$\pm$0.47 &  & 98.0$\pm$10.7 & 0.15$\pm$0.49 &  \\
Bone\_Vert\_C3 & 98.1$\pm$23.4 & 0.16$\pm$3.22 & 98.1$\pm$23.4 & 0.16$\pm$3.22 & 94.8$\pm$10.3 & 0.28$\pm$0.64 & 98.0$\pm$15.5 & 0.16$\pm$3.18 &  & 92.1$\pm$15.5 & 0.33$\pm$3.05 &  & 98.2$\pm$15.4 & 0.15$\pm$2.86 &  \\
Bone\_Vert\_C4 & 97.0$\pm$23.4 & 0.34$\pm$3.60 & 97.0$\pm$23.4 & 0.34$\pm$3.60 & 92.1$\pm$20.0 & 0.60$\pm$1.99 & 96.6$\pm$19.6 & 0.30$\pm$3.54 &  & 85.4$\pm$19.5 & 0.30$\pm$3.26 &  & 95.9$\pm$19.5 & 0.27$\pm$3.36 &  \\
Bone\_Vert\_C5 & 96.8$\pm$17.5 & 0.22$\pm$1.62 & 96.8$\pm$17.5 & 0.22$\pm$1.62 & 88.7$\pm$22.3 & 0.26$\pm$0.62 & 97.8$\pm$17.4 & 0.21$\pm$1.63 &  & 86.2$\pm$17.4 & 0.39$\pm$1.48 &  & 97.8$\pm$17.3 & 0.19$\pm$1.49 &  \\
Bone\_Vert\_C6 & 95.0$\pm$10.6 & 0.60$\pm$0.93 & 95.0$\pm$10.6 & 0.60$\pm$0.93 & 96.9$\pm$4.6 & 0.16$\pm$0.33 & 96.0$\pm$10.5 & 0.45$\pm$0.93 &  & 85.9$\pm$10.4 & 0.45$\pm$0.92 &  & 95.1$\pm$10.5 & 0.44$\pm$0.93 &  \\
Bone\_Vert\_C7 & 95.2$\pm$17.5 & 0.41$\pm$0.86 & 95.2$\pm$17.5 & 0.41$\pm$0.86 & 96.5$\pm$5.8 & 0.19$\pm$0.45 & 95.3$\pm$13.1 & 0.18$\pm$1.00 &  & 93.9$\pm$13.3 & 0.30$\pm$0.97 &  & 96.1$\pm$13.0 & 0.19$\pm$0.98 &  \\
Bone\_Vert\_L1 & 95.7$\pm$12.1 & 1.27$\pm$0.98 & 95.7$\pm$12.1 & 1.27$\pm$0.98 & 97.1$\pm$3.1 & 0.14$\pm$0.30 & 94.9$\pm$12.1 & 1.19$\pm$0.98 &  & 94.9$\pm$12.1 & 1.15$\pm$0.99 &  & 94.4$\pm$12.0 & 1.13$\pm$0.97 &  \\
Bone\_Vert\_L2 & 94.8$\pm$18.2 & 0.29$\pm$1.09 & 94.8$\pm$18.2 & 0.29$\pm$1.09 & 97.4$\pm$1.7 & 0.11$\pm$0.21 & 93.7$\pm$12.3 & 0.18$\pm$0.95 &  & 97.0$\pm$12.4 & 0.12$\pm$0.96 &  & 92.8$\pm$12.1 & 0.18$\pm$0.93 &  \\
Bone\_Vert\_L3 & 96.0$\pm$16.1 & 0.24$\pm$1.09 & 96.0$\pm$16.1 & 0.24$\pm$1.09 & 97.0$\pm$1.8 & 0.13$\pm$0.16 & 96.9$\pm$16.2 & 0.18$\pm$1.06 &  & 96.9$\pm$16.2 & 0.27$\pm$1.02 &  & 97.3$\pm$16.3 & 0.20$\pm$0.96 &  \\
Bone\_Vert\_L4 & 94.1$\pm$14.3 & 0.43$\pm$0.41 & 94.1$\pm$14.3 & 0.43$\pm$0.41 & 95.7$\pm$6.4 & 0.22$\pm$0.39 & 94.2$\pm$14.2 & 0.23$\pm$0.41 &  & 96.1$\pm$14.0 & 0.20$\pm$0.39 &  & 94.6$\pm$14.0 & 0.24$\pm$0.39 &  \\
Bone\_Vert\_L5 & 92.9$\pm$17.3 & 0.21$\pm$1.49 & 92.9$\pm$17.3 & 0.21$\pm$1.49 & 94.6$\pm$9.5 & 0.31$\pm$0.70 & 93.9$\pm$17.4 & 0.19$\pm$1.43 &  & 97.1$\pm$17.4 & 0.32$\pm$1.38 &  & 93.9$\pm$17.2 & 0.18$\pm$1.40 &  \\
Bone\_Vert\_S1 & 96.3$\pm$23.8 & 0.20$\pm$2.10 & 96.3$\pm$23.8 & 0.20$\pm$2.10 & 92.0$\pm$14.2 & 0.42$\pm$0.96 & 97.3$\pm$18.9 & 0.19$\pm$1.22 &  & 97.4$\pm$19.0 & 1.08$\pm$1.16 &  & 97.3$\pm$19.0 & 0.18$\pm$1.12 &  \\
Bone\_Vert\_T1 & 96.3$\pm$23.5 & 0.15$\pm$1.28 & 96.3$\pm$23.5 & 0.15$\pm$1.28 & 92.5$\pm$13.0 & 0.41$\pm$0.94 & 95.9$\pm$13.5 & 0.15$\pm$1.37 &  & 95.6$\pm$13.6 & 0.23$\pm$1.25 &  & 96.8$\pm$13.6 & 0.14$\pm$1.25 &  \\
Bone\_Vert\_T2 & 98.0$\pm$5.2 & 0.48$\pm$0.74 & 98.0$\pm$5.2 & 0.48$\pm$0.74 & 88.6$\pm$22.0 & 0.59$\pm$1.38 & 97.7$\pm$5.4 & 0.32$\pm$0.76 &  & 90.2$\pm$5.5 & 0.82$\pm$0.76 &  & 97.5$\pm$5.6 & 0.32$\pm$0.77 &  \\
Bone\_Vert\_T3 & 97.0$\pm$2.7 & 0.48$\pm$0.20 & 97.0$\pm$2.7 & 0.48$\pm$0.20 & 90.4$\pm$17.1 & 0.64$\pm$1.58 & 97.9$\pm$2.6 & 0.46$\pm$0.21 &  & 88.5$\pm$2.7 & 1.10$\pm$0.22 &  & 97.9$\pm$2.5 & 0.44$\pm$0.20 &  \\
Bone\_Vert\_T4 & 89.6$\pm$17.0 & 1.12$\pm$0.21 & 89.6$\pm$17.0 & 1.12$\pm$0.21 & 91.2$\pm$16.9 & 0.51$\pm$1.50 & 90.5$\pm$8.9 & 1.05$\pm$0.20 &  & 87.7$\pm$9.0 & 1.12$\pm$0.21 &  & 91.4$\pm$8.9 & 0.95$\pm$0.20 &  \\
Bone\_Vert\_T5 & 90.7$\pm$22.9 & 0.92$\pm$0.38 & 90.7$\pm$22.9 & 0.92$\pm$0.38 & 93.6$\pm$15.8 & 0.42$\pm$1.73 & 90.4$\pm$23.1 & 0.88$\pm$0.39 &  & 92.7$\pm$23.1 & 0.62$\pm$0.39 &  & 91.0$\pm$22.9 & 0.97$\pm$0.37 &  \\
Bone\_Vert\_T6 & 86.3$\pm$28.3 & 1.15$\pm$0.07 & 86.3$\pm$28.3 & 1.15$\pm$0.07 & 92.8$\pm$15.8 & 0.48$\pm$2.13 & 85.4$\pm$28.1 & 1.04$\pm$0.06 &  & 95.2$\pm$28.0 & 0.54$\pm$0.05 &  & 85.4$\pm$28.2 & 0.94$\pm$0.06 &  \\
Bone\_Vert\_T7 & 96.8$\pm$1.0 & 1.58$\pm$0.04 & 96.8$\pm$1.0 & 1.58$\pm$0.04 & 89.9$\pm$17.5 & 0.37$\pm$1.00 & 97.1$\pm$1.0 & 1.48$\pm$0.06 &  & 93.2$\pm$1.0 & 0.34$\pm$0.05 &  & 97.0$\pm$1.2 & 1.62$\pm$0.08 &  \\
Bone\_Vert\_T8 & 91.5$\pm$13.0 & 1.08$\pm$0.40 & 91.5$\pm$13.0 & 1.08$\pm$0.40 & 84.9$\pm$24.3 & 0.18$\pm$0.22 & 91.6$\pm$13.0 & 0.93$\pm$0.16 &  & 95.4$\pm$13.1 & 0.24$\pm$0.17 &  & 91.9$\pm$13.0 & 1.00$\pm$0.17 &  \\
Bone\_Vert\_T9 & 94.6$\pm$44.2 & 0.53$\pm$0.23 & 94.6$\pm$44.2 & 0.53$\pm$0.23 & 94.4$\pm$4.6 & 0.08$\pm$0.03 & 94.3$\pm$14.4 & 0.42$\pm$0.24 &  & 94.2$\pm$14.5 & 0.47$\pm$0.26 &  & 93.3$\pm$14.4 & 0.46$\pm$0.25 &  \\
Bone\_Vert\_T10 & 97.6$\pm$29.9 & 0.36$\pm$2.18 & 97.6$\pm$29.9 & 0.36$\pm$2.18 & 95.8$\pm$0.9 & 0.10$\pm$0.07 & 97.5$\pm$13.0 & 0.38$\pm$1.32 &  & 93.3$\pm$12.9 & 0.31$\pm$1.19 &  & 97.4$\pm$13.0 & 0.37$\pm$1.21 &  \\
Bone\_Vert\_T11 & 95.1$\pm$19.4 & 0.25$\pm$1.64 & 95.1$\pm$19.4 & 0.25$\pm$1.64 & 94.7$\pm$5.5 & 0.22$\pm$0.46 & 95.1$\pm$12.4 & 0.22$\pm$1.67 &  & 93.8$\pm$12.4 & 0.37$\pm$1.62 &  & 95.6$\pm$12.4 & 0.23$\pm$1.64 &  \\
Bone\_Vert\_T12 & 97.2$\pm$16.3 & 0.32$\pm$1.30 & 97.2$\pm$16.3 & 0.32$\pm$1.30 & 84.3$\pm$27.3 & 0.24$\pm$0.34 & 97.5$\pm$16.0 & 0.26$\pm$1.35 &  & 90.5$\pm$15.9 & 1.16$\pm$1.30 &  & 97.7$\pm$16.1 & 0.24$\pm$1.26 & 

 \\ \hline
\end{tabular}}
\caption{\ac{pl} performance details: Organ-wise TotalSegmentator -- `Vertebrae' subgroup}
\end{table}

==> Tabs/tabs_external/tab_external_abdomen_btcv_clnet_nn.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|ll|ll|ll|}
\hline
 & \multicolumn{2}{c|}{\ac{nnu_e36}} & \multicolumn{2}{c|}{\ac{cln_c36}} & \multicolumn{2}{c|}{\ac{cln_u36}} \\ \cline{2-7} 
\multirow{-2}{*}{} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} \\ \hline
\rowcolor[HTML]{F3F3F3} 
Spleen & 93.4$\pm$6.9 & 0.74$\pm$0.49 & 94.7$\pm$7.7 & 0.71$\pm$0.51 & 94.3$\pm$6.0 & 0.57$\pm$0.54 \\
Kidney\_R & 91.0$\pm$7.0 & 0.62$\pm$0.74 & 91.2$\pm$6.7 & 0.78$\pm$0.85 & 91.3$\pm$6.5 & 0.73$\pm$0.62 \\
Kidney\_L & 91.2$\pm$6.8 & 0.83$\pm$0.77 & 91.0$\pm$7.6 & 1.61$\pm$0.62 & 91.7$\pm$8.3 & 1.73$\pm$0.75 \\
\rowcolor[HTML]{F3F3F3} 
Gallbladder & 71.3$\pm$8.7 & 1.90$\pm$0.82 & 72.0$\pm$9.6 & 1.27$\pm$0.79 & 72.8$\pm$8.7 & 1.41$\pm$0.79 \\
Eso & 79.0$\pm$9.6 & 1.68$\pm$1.33 & 80.1$\pm$10.5 & 1.38$\pm$1.41 & 81.1$\pm$10.6 & 1.26$\pm$1.36 \\
\rowcolor[HTML]{F3F3F3} 
Liver & 97.0$\pm$0.5 & 0.79$\pm$1.03 & 96.4$\pm$0.4 & 1.21$\pm$1.00 & 97.3$\pm$0.7 & 1.24$\pm$0.95 \\
Stomach & 89.6$\pm$8.6 & 1.26$\pm$0.99 & 86.8$\pm$9.6 & 1.53$\pm$0.98 & 87.8$\pm$9.5 & 1.48$\pm$0.95 \\
\rowcolor[HTML]{F3F3F3} 
A\_Aorta & 91.1$\pm$3.6 & 1.51$\pm$0.36 & 92.2$\pm$4.2 & 1.31$\pm$0.34 & 92.5$\pm$4.2 & 1.19$\pm$0.28 \\
V\_VenaCava\_I & 88.0$\pm$7.0 & 2.03$\pm$0.49 & 86.8$\pm$6.4 & 1.92$\pm$0.56 & 86.3$\pm$6.4 & 1.81$\pm$0.53 \\
\rowcolor[HTML]{F3F3F3} 
V\_Portal\_Splenic & 77.0$\pm$19.0 & 1.48$\pm$0.79 & 75.9$\pm$19.9 & 1.71$\pm$0.73 & 75.8$\pm$19.2 & 1.74$\pm$0.74 \\
Pancreas & 83.4$\pm$9.2 & 1.53$\pm$0.37 & 82.2$\pm$10.1 & 1.56$\pm$0.33 & 81.9$\pm$7.3 & 1.48$\pm$0.38 \\
\rowcolor[HTML]{F3F3F3} 
Glnd\_Adrenal\_R & 72.1$\pm$14.2 & 1.30$\pm$0.43 & 75.1$\pm$14.9 & 0.89$\pm$0.46 & 76.0$\pm$16.0 & 0.76$\pm$0.50 \\
\rowcolor[HTML]{F3F3F3} 
Glnd\_Adrenal\_L & 72.0$\pm$16.4 & 1.67$\pm$0.45 & 75.0$\pm$17.3 & 0.89$\pm$0.46 & 75.4$\pm$17.1 & 0.95$\pm$0.51 \\ \hline
Mean & \multicolumn{1}{c}{84.32} & \multicolumn{1}{c|}{1.33} & \multicolumn{1}{c}{84.57} & \multicolumn{1}{c|}{1.29} & \multicolumn{1}{c}{84.94} & \multicolumn{1}{c|}{1.26} \\ \hline
\end{tabular}}
\caption{\textbar\textbf{External testing: Organ-wise segmentation performance comparison on  160 patients chest dataset}. The organ-wise DSC (\%) and ASD (mm) are evaluated for comparison.  The \ac{cln_u36} achieves the best mean DSC and ASD. }
\label{tab:external_abdomen}
\end{table}

==> Tabs/tabs_external/tab_external_chest_clnet_nn.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|ll|ll|ll|}
\hline
 & \multicolumn{2}{c|}{\ac{nnu_e36}} & \multicolumn{2}{c|}{\ac{cln_c36}} & \multicolumn{2}{c|}{\ac{cln_u36}} \\ \cline{2-7} 
\multirow{-2}{*}{} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} \\ \hline

\rowcolor[HTML]{F3F3F3} 
BrachialPlex & 40.5$\pm$11.8 & 3.35$\pm$3.69 & 49.0$\pm$8.8 & 2.52$\pm$2.88 & 49.9$\pm$8.8 & 2.54$\pm$2.09 \\
Eso & 84.3$\pm$6.6 & 1.12$\pm$0.68 & 88.3$\pm$5.8 & 0.68$\pm$0.68 & 88.3$\pm$5.3 & 0.70$\pm$0.70 \\
\rowcolor[HTML]{F3F3F3} 
Lung\_L & 98.0$\pm$0.4 & 0.85$\pm$1.07 & 98.1$\pm$0.4 & 0.84$\pm$0.99 & 98.2$\pm$0.6 & 0.68$\pm$1.35 \\
\rowcolor[HTML]{F3F3F3} 
Lung\_R & 97.0$\pm$0.4 & 0.80$\pm$1.02 & 97.1$\pm$0.3 & 0.80$\pm$0.54 & 97.8$\pm$0.6 & 0.60$\pm$1.10 \\
Pericardium & 92.2$\pm$1.8 & 1.62$\pm$3.84 & 92.2$\pm$1.4 & 1.62$\pm$3.69 & 92.4$\pm$1.8 & 1.54$\pm$4.45 \\
\rowcolor[HTML]{F3F3F3} 
SpinalCord & 89.5$\pm$3.4 & 1.13$\pm$1.16 & 91.8$\pm$2.5 & 0.90$\pm$0.85 & 92.2$\pm$2.3 & 0.85$\pm$0.86 \\
ProximalBronchi & 91.0$\pm$2.3 & 0.89$\pm$0.75 & 91.1$\pm$1.9 & 0.89$\pm$0.70 & 91.5$\pm$2.0 & 0.88$\pm$0.67 \\
\rowcolor[HTML]{F3F3F3} 
A\_Aorta & 92.0$\pm$7.5 & 1.34$\pm$4.42 & 92.8$\pm$7.7 & 1.11$\pm$4.63 & 92.9$\pm$8.0 & 1.03$\pm$4.65 \\
A\_Pulmonary & 87.8$\pm$4.0 & 1.12$\pm$1.47 & 87.8$\pm$4.0 & 1.10$\pm$1.09 & 89.0$\pm$3.8 & 0.88$\pm$1.44 \\
\rowcolor[HTML]{F3F3F3} 
V\_Pulmonary & 69.7$\pm$9.5 & 2.21$\pm$1.24 & 71.2$\pm$8.0 & 1.94$\pm$0.99 & 73.3$\pm$8.2 & 1.80$\pm$1.43 \\
V\_Venacava\_I & 88.0$\pm$7.6 & 1.22$\pm$1.10 & 86.3$\pm$7.5 & 1.16$\pm$1.10 & 88.6$\pm$8.1 & 0.95$\pm$1.15 \\
\rowcolor[HTML]{F3F3F3} 
V\_Venacava\_S & 86.2$\pm$4.1 & 1.09$\pm$0.87 & 87.8$\pm$4.2 & 0.88$\pm$0.52 & 87.9$\pm$4.4 & 0.86$\pm$0.68 \\
ChestWall\_L & 90.2$\pm$2.3 & 1.45$\pm$0.98 & 90.4$\pm$2.2 & 1.03$\pm$0.99 & 90.9$\pm$2.6 & 1.23$\pm$1.20 \\
ChestWall\_R & 90.3$\pm$2.0 & 1.13$\pm$0.89 & 90.9$\pm$2.0 & 0.99$\pm$0.88 & 90.8$\pm$2.1 & 0.64$\pm$0.50 \\ \hline
Mean & \multicolumn{1}{c}{85.48} & \multicolumn{1}{c|}{1.38} & \multicolumn{1}{c}{86.77} & \multicolumn{1}{c|}{1.18} & \multicolumn{1}{c}{87.41} & \multicolumn{1}{c|}{1.08} \\ \hline
\end{tabular}}
\caption{\textbf{External testing: organ-wise segmentation performance comparison on  160 patients chest dataset}. The dataset-wise DSC (\%) and ASD (mm) of \ac{nnu_e36}, \ac{cln_c36} and \ac{cln_u36}. \ac{cln_u36} achieves the best mean DSC and ASD. }
\label{tab:external_chest}
\end{table}

==> Tabs/tabs_external/tab_external_hn_clnet_nn.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|ll|ll|ll|}
\hline
 & \multicolumn{2}{c|}{\ac{nnu_e36}} & \multicolumn{2}{c|}{\ac{cln_c36}} & \multicolumn{2}{c|}{\ac{cln_u36}} \\ \cline{2-7} 
\multirow{-2}{*}{} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} \\ \hline
\rowcolor[HTML]{F3F3F3} 
BrainStem & 85.3$\pm$4.6 & 1.20$\pm$0.49 & 85.1$\pm$4.1 & 1.02$\pm$0.53 & 85.7$\pm$3.6 & 0.96$\pm$0.50 \\
Eye\_L & 89.2$\pm$5.2 & 0.71$\pm$0.40 & 89.5$\pm$2.7 & 0.46$\pm$0.16 & 89.2$\pm$2.8 & 0.48$\pm$0.17 \\
Eye\_R & 89.3$\pm$3.6 & 0.69$\pm$0.29 & 88.7$\pm$2.7 & 0.53$\pm$0.18 & 89.1$\pm$2.5 & 0.50$\pm$0.17 \\
\rowcolor[HTML]{F3F3F3} 
Lens\_L & 74.5$\pm$7.9 & 0.48$\pm$0.24 & 75.1$\pm$10.1 & 0.57$\pm$0.39 & 75.8$\pm$8.6 & 0.53$\pm$0.32 \\
\rowcolor[HTML]{F3F3F3} 
Lens\_R & 72.7$\pm$10.1 & 0.52$\pm$0.31 & 75.0$\pm$11.6 & 0.60$\pm$0.39 & 75.4$\pm$8.7 & 0.52$\pm$0.33 \\
Chiasm & 50.5$\pm$13.1 & 1.42$\pm$0.66 & 54.6$\pm$12.3 & 0.82$\pm$0.59 & 54.6$\pm$12.2 & 0.82$\pm$0.63 \\
\rowcolor[HTML]{F3F3F3} 
OpticNerve\_L & 68.0$\pm$9.3 & 0.79$\pm$0.38 & 68.2$\pm$10.4 & 0.56$\pm$0.34 & 69.7$\pm$9.7 & 0.58$\pm$0.35 \\
\rowcolor[HTML]{F3F3F3} 
OpticNerve\_R & 67.4$\pm$11.1 & 0.84$\pm$0.48 & 69.4$\pm$8.7 & 0.59$\pm$0.41 & 69.2$\pm$7.9 & 0.61$\pm$0.47 \\
Glnd\_Parotid\_L & 84.2$\pm$5.8 & 1.23$\pm$0.73 & 85.6$\pm$3.9 & 1.05$\pm$0.35 & 85.8$\pm$3.5 & 0.99$\pm$0.29 \\
Glnd\_Parotid\_R & 83.9$\pm$5.6 & 1.27$\pm$0.53 & 85.7$\pm$3.5 & 1.09$\pm$0.39 & 85.8$\pm$3.5 & 1.05$\pm$0.39 \\
\rowcolor[HTML]{F3F3F3} 
TMJ\_L & 69.8$\pm$11.5 & 1.07$\pm$0.53 & 72.2$\pm$12.0 & 0.89$\pm$0.57 & 72.4$\pm$9.3 & 0.63$\pm$0.48 \\
\rowcolor[HTML]{F3F3F3} 
TMJ\_R & 69.6$\pm$12.3 & 1.10$\pm$0.58 & 71.5$\pm$12.6 & 0.94$\pm$0.58 & 71.9$\pm$10.7 & 0.67$\pm$0.52 \\ \hline
Mean & \multicolumn{1}{c}{75.37} & \multicolumn{1}{c|}{0.94} & \multicolumn{1}{c}{76.72} & \multicolumn{1}{c|}{0.76} & \multicolumn{1}{c}{77.05} & \multicolumn{1}{c|}{0.70} \\ \hline
\end{tabular}}
\caption{\textbf{External testing: Organ-wise segmentation performance comparison on  160 patients chest dataset}.  The dataset-wise DSC (\%) and ASD (mm) of  \ac{nnu_e36}, \ac{cln_c36} and \ac{cln_u36}. \ac{cln_u36} achieves the best mean DSC and ASD. }
\label{tab:external_hn}
\end{table}

==> Tabs/tabs_external/tab_external_lesion_clnet_nn.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|ll|ll|ll|}
\hline
 & \multicolumn{2}{c|}{\ac{nnu_e36}} & \multicolumn{2}{c|}{\ac{cln_c36}} & \multicolumn{2}{c|}{\ac{cln_u36}} \\ \cline{2-7} 
\multirow{-2}{*}{} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} & \multicolumn{1}{c}{DSC$\uparrow$} & \multicolumn{1}{c|}{ASD$\downarrow$} \\ \hline
\rowcolor[HTML]{F3F3F3} 
\ac{npc}\_\Ac{gtv} & 70.3$\pm$13.1 & 2.02$\pm$1.46 & 70.5$\pm$14.2 & 2.01$\pm$1.59 & 70.3$\pm$9.9 & 1.98$\pm$1.58 \\

Eso\_\Ac{gtv} & 75.0$\pm$18.4 & 8.85$\pm$14.23 & 74.9$\pm$16.7 & 8.87$\pm$12.24 & 75.1$\pm$18.8 & 8.67$\pm$14.50 \\

\rowcolor[HTML]{F3F3F3} 
Liver\_\Ac{gtv} & 69.9$\pm$16.3 & 8.41$\pm$4.31 & 69.9$\pm$20.9 & 8.43$\pm$6.42 & 70.4$\pm$18.1 & 7.53$\pm$4.74 \\ 

Kidney\_\Ac{gtv} & 83.6$\pm$18.1 & 2.20$\pm$1.64 & 86.6$\pm$12.6 & 1.01$\pm$0.99 & 86.7$\pm$11.0 & 1.00$\pm$0.99 \\ \hline
Mean & \multicolumn{1}{c}{74.70} & \multicolumn{1}{c|}{5.37} & \multicolumn{1}{c}{75.48} & \multicolumn{1}{c|}{5.08} & \multicolumn{1}{c}{75.63} & \multicolumn{1}{c|}{4.80} \\ \hline
\end{tabular}}
\caption{\textbf{External testing: Organ-wise segmentation performance comparison on external 319 \ac{npc} \ac{gtv} patients, 148 Eso \ac{gtv} patients, 176 Liver \ac{gtv} patients, and 978 Kidney \ac{gtv} patients}. The dataset-wise DSC (\%) and ASD (mm) of  \ac{nnu_e36}, \ac{cln_c36} and \ac{cln_u36}. \ac{cln_c36} achieves the best mean DSC and ASD. }
\label{tab:external_lesion}
\end{table}

==> Tabs/tabs_external/tab_external_summary_clnet_nn_v2.tex <==

\begin{table}[htp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}clcccccc|c@{}}
\toprule
\textbf{Metric} &
  \textbf{Method} &
  \textbf{HeadNeck\_GZ\_12 } &
  \textbf{Chest\_ZJU\&SH\_14} &
  \textbf{BTCV} &
  \textbf{HeadNeck\_CGMH-NPC\_1} &
  \textbf{Chest\_CGMH-EsoCancer\_1} &
  \textbf{Abdomen\_CGMH-LiverCancer\_1} &
  \textbf{Mean} \\ \midrule
 &
  \ac{nnu_e36} &
  75.37 &
  85.48 &
  84.32 &
  70.35 &
  75.01 &
  69.90 &
  81.25 \\
 &
  \ac{cln_c36} &
  76.72 &
  86.77 &
  84.57 &
  \textbf{74.47} &
  \textbf{74.90} &
  \textbf{70.40} &
  82.16 \\
\multirow{-3}{*}{DSC$\uparrow$} &
  \ac{cln_u36} &
  \textbf{77.05} &
  \textbf{87.41} &
  \textbf{84.94} &
  70.30 &
  75.11 &
  69.87 &
  \textbf{82.57} \\ \midrule
 &
  \ac{nnu_e36} &
  0.94 &
  1.38 &
  1.72 &
  2.02 &
  8.85 &
  8.41 &
  1.72 \\
 &
  \ac{cln_c36} &
  0.76 &
  1.18 &
  1.63 &
  \textbf{2.01} &
  \textbf{8.87} &
  \textbf{7.53} &
  1.55 \\

\multirow{-4}{*}{ASD$\downarrow$} &
  \ac{cln_u36} &
  \textbf{0.70} &
  \textbf{1.08} &
  \textbf{1.61} &
  1.98 &
  8.67 &
  8.43 &
  \textbf{1.51} \\ \bottomrule
\end{tabular}%
}
\caption{\textbar~\textbf{Performance comparison of \ac{nnu_e36}, \ac{cln_c36} and \ac{cln_u36} on six external testing datasets.} The mean DSC (\%) and ASD (mm) are evaluated on different body parts. \ac{cln_u36} achieves the top performance in both DSC and ASD.  }
\label{tab:pl_ex_res_main} % not use in paper
\end{table}

==> discussion/discussion_insight.tex <==
% Dataset Settings
% \begin{itemize}
%     \item Public Dataset: Enable large-scale model training under partial label supervision but may have inconsistent annotation styles due to different sources. The predominance of healthy organs limits the datasets' representation of real-world clinical scenarios, affecting segmentation diversity and robustness; 
    
%     \item Private Dataset: Focus on disease-oriented cases. Expert-reviewed labels ensure consistency. Privacy-controlled, requiring model training at different sites, making performance sensitive to the learning sequence; 
    
%     \item Figure--Dataset: Introduce dataset fingerprints, especially body part regression (BPR). Datasets are grouped by the corresponding body part; 
% \end{itemize}

% Validation Experiment Settings
% \begin{itemize}
%     \item Motivation: Conducting all experiments on full-scale datasets is computationally expensive, time-consuming, and impractical. Some comparison methods are unsuitable for large datasets. Thus, designed a small-scale validation using 5 public datasets -> efficient and comprehensive evaluation. 

%     \item \ac{css} protocol: Only the current dataset available for training and pruning, while previous datasets remain inaccessible. To thoroughly evaluate segmentation performance, forgetting rate, and order sensitivity, four dataset orders (O1-O4) for \ac{css} setting. O1-O4 vary based on body part or organ type, allowing the investigation of the impact of order on \ac{clnet} performance. The comparison between O1 and O2 helps assess order sensitivity, as both share the same initial step. 

%     \item Ablation study: Explore the impact of the decoder pruning process on segmentation accuracy and model size. Model scale and parameter growth rate are the major challenges in architecture-based \ac{css} method. 

%     \item \ac{pl} protocol: With rapid growth of public medical datasets, it's valuable to explore \ac{clnet} ability in \ac{pl} setting. All training datasets are accessible simultaneously, each partially annotating target organs. Train a unified model with integrated medical knowledge and potentially better performance. 
% \end{itemize}

% Full-scale Experiment Settings
% \begin{itemize}
%     \item Motivation: train a lifelong, unified model, generalizability and scalability, segments a wide range of whole-body organs, extended to new tasks. 

%     \item \ac{css} protocol, \ac{pl} protocol, Decoder pruning: similar to Validation Experimental Setting. 
% \end{itemize}

% Validation CSS Discussion
% \begin{itemize}
%     \item \Ac{clnet} outperforms other leading methods across all datasets under various orders, and shows performance on par with or even surpass the nnUNet upper bound performance. It reveals that our general encoder is able to guarantee the top-level segmentation performance even without finetuning. 

%     \item \ac{clnet} shows advantages in both model stability and plasticity, which plays significant roles and trade-off in continual learning and segmentation, i.e. a stable model resists catastrophic forgetting, while a plastic model learns better on new tasks. 
%     \begin{itemize}
%         \item The advanced model stability of \ac{clnet} is mainly supported by its non-forgetting ability. (flat forgetting curve) In comparison, other methods have mainly decreasing curves, and some recovery curves are due to rehearsal from overlapping organs. 

%         \item \Ac{clnet} exhibits superior plasticity due to the general and robust visual features from its frozen \ac{ge} and incrementally added decoder heads for knowledge updates. CLNet reaches the nnUNet performance upper bound on sequential datasets, showcasing its strong plasticity. In contrast, comparison methods suffer from reduced plasticity due to their knowledge-distillation strategies, which prioritize stability and forgetting prevention but hinder adaptation to new tasks. 
%     \end{itemize}

%     \item \Ac{clnet} achieves top organ segmentation performance while maintaining a tiny model size and low parameter growth. In real-world deployment, both prediction accuracy and model size are crucial for CSS methods. After continual learning, \ac{clnet}'s lower parameter size and higher DSC indicate superior performance, and its stable results across all CSS orders also demonstrate robustness to order variations. 
% \end{itemize}

% Validation Ablation Study Discussion
% \begin{itemize}
%     \item The decoder pruning process effectively maintains \ac{clnet} performance while efficiently reduces the model size.

%     \item Motivation and scale law: balancing model scale and accuracy is crucial to avoid excessive physical storage and GPU memory costs.  Significant in architecture-based \ac{css} method (\ac{clnet}): incremental decoder expansion can lead to rapid model growth and parameter explosion. Thus, decoder pruning. 

%     \item Ablation of other key modules. (@Dazhou)
% \end{itemize}

% Full-scale CSS Discussion
% \begin{itemize}
%     \item Compared to \ac{nnu_e36}, \ac{cln_c36} achieves comparable or superior results on all \ac{orgn} organs and better mean DSC on each organ group. Demonstrate the advanced accuracy, generalizability, robustness, strong scalability and non-forgettable learning ability of \ac{clnet} under \ac{css} situation. 

%     \item Most chest, abdomen and bone organs have higher dice scores with moderate variations, probably due to the large size, stable shape and relative fixed anatomical position of these organs; Head-neck, LNS and \ac{gtv} organs as well as some vessels from chest have small size, complex or irregular shape, and diverse location,  resulting in relative lower DSCs with wide variations. 

%     \item The remarkably boosted segmentation performance on head-neck and chest groups reveals that \ac{clnet} has particular advantages in segmenting tiny and complicated organs such as head \& neck substructures, nerves, blood vessels, and bronchi. 
% \end{itemize}

==> discussion/discussion_limitation.tex <==
% Validation PL Discussion
% \begin{itemize}
%     \item \Ac{clnet} can be smoothly expanded to \ac{pl} setting with slightly better segmentation performance than \ac{cln_c5}. 

%     \item Unlike the practical \ac{css} setting, \ac{pl} is actually an easier setting where the limitation of dataset accessibility is released so that all datasets can be trained simultaneously. 

%     \item \ac{cln_c5} closely reaches the \ac{pl} upper bound. 
    
%     \item Better performance than leading \ac{pl} method -- Multi-talent. 
% \end{itemize}

% Full-scale PL Discussion
% \begin{itemize}
%     \item Compared to \ac{cln_c36}, \ac{cln_u36} enhances segmentation performance with a modest improvement, and subtle performance fluctuation on each organ. 

%     \item The performance gap between \ac{css} and \ac{pl} is not significant, indicating that \ac{cln_c36} may be approaching the upper bound of large-scale whole-body organ segmentation. 
% \end{itemize}

% Full-scale Decoder Pruning Discussion
% \begin{itemize}
%     \item Decoder pruning: validate the effectiveness of model compression and the potential influence on segmentation performance.

%     \item The decoder pruning process effectively reduces the parameter size of all decoder heads, limiting parameter growth on new tasks.  The high and stable pruning rate across \ac{orgn} whole-body organs its effectiveness in controlling model scale and preventing parameter explosion, a common issue in architecture-based CSS methods. 

%     \item The \ac{clnet} decoders after extensive pruning can still keep and even slightly improves the overall segmentation performance. Since a deep model with a large number of parameters is prone to overfitting the training data including noise and outliers, the modest performance enhancement after pruning is likely due to the reduced overfitting achieved by removing redundant parameters during the pruning process. 
    
%     \item Most of the decoders (except \ac{gtv} group) have less than $\pm$0.1\% $\Delta$DSC. The marginally reduced performance of some decoders in \ac{gtv} group is probably caused by the pruned parameters that are related to the detailed features for the diverse location and complex appearance of the \ac{gtv}s. 
% \end{itemize}

==> discussion/discussion_method.tex <==
%Using \ac{ema} can help stabilize the fine-tuning process and learn more robust features by reducing the impact of abrupt gradient changes. The \ac{ema} update works effectively when the input body part and output classes of the decoding path remain consistent. However, a potential drawback arises when different decoders with varying output classes are sequentially used for \ac{ge} updates. In such cases, \ac{ema} might not effectively `preserve' previously learned features but smooth out the distinctive features of each task on-the-fly. This smoothing effect can blur the specific characteristics unique to each task, potentially reducing the \ac{ge}'s ability to accurately capture the finer details necessary for distinguishing between different body parts and segmentation classes. 
